Not All Steps are Created Equal: Selective Diffusion Distillation for Image Manipulation

Conditional diffusion models have demonstrated impressive performance in image manipulation tasks. The general pipeline involves adding noise to the image and then denoising it. However, this method faces a trade-off problem: adding too much noise affects the fidelity of the image while adding too little affects its editability. This largely limits their practical applicability. In this paper, we propose a novel framework, Selective Diffusion Distillation (SDD), that ensures both the fidelity and editability of images. Instead of directly editing images with a diffusion model, we train a feedforward image manipulation network under the guidance of the diffusion model. Besides, we propose an effective indicator to select the semantic-related timestep to obtain the correct semantic guidance from the diffusion model. This approach successfully avoids the dilemma caused by the diffusion process. Our extensive experiments demonstrate the advantages of our framework. Code is released at https://github.com/AndysonYs/Selective-Diffusion-Distillation.

==> latexmkrc <==
add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );

sub makeexternaldocument {
    # if the dependency isn't one of the files that this latexmk run will consider, process it
    # without this test, we would get an infinite loop!
    if (!($root_filename eq $_[0]))
    {   # PLEASE ENABLE ONLY ONE OF THE FOLLOWING
        # DEPENDING ON THE ENGINE YOU'RE USING
    
        # FOR PDFLATEX
        system( "latexmk -pdf \"$_[0]\"" );

        # FOR LATEX+DVIPDF
        # system( "latexmk \"$_[0]\"" );

        # FOR XELATEX
        # system( "latexmk -xelatex \"$_[0]\"" );
        
        # FOR LUALATEX
        # system( "latexmk -lualatex \"$_[0]\"" );
   }
}


==> legacy/00_abstract.tex <==
\begin{abstract}
% Abstract goes here.
Diffusion models have achieved impressive performance on the image generation task. This urges computer scientists to extend it to image editing. However, existing image editing methods all rely on the iterative denoising process, hence the editing speed is pretty slow. 
In this work, we propose a novel image editing paradigm by using diffusion model loss as guidance. With this new paradigm, we avoid the expensive time consumption during inference while benefiting from the remarkable generation quality of the diffusion model. Besides, we also observe that our method is susceptible to the choice of training timestep. Therefore, we propose an entropy-based step-pruning strategy to further improve the performance of our method. We conduct extended experiments to demonstrate the high-quality and efficiency of our method in a wide range of image editing tasks.
% The implementation is available at  \url{https://github.com/AndysonYs/Image-Editing-by-Diffusion-Prior}. 
\end{abstract}

==> legacy/01_intro.tex <==
\section{Introduction}
\label{sec:intro}
%%%%  Background: The diffusion model is a strong prior model
Diffusion models have achieved an overwhelming performance on the image generation task. Among these tasks, guided image editing has become popular since it can guide the source image to the target direction without changing other preserved properties. 
Recently, diffusion models conditioned on natural language text prompts\cite{saharia2022imagen, rombach2022stablediffusion, nichol2021glide, ramesh2022dalle2} have shown their ability of diverse and controllable image synthesis. The promising results further spur computer scientists to fully utilize the diffusion model in the text-guidance image editing task.

Conventional methods\cite{choi2021ilvr,meng2021sdedit,avrahami2022blended,zhao2022egsde, dhariwal2021guided} are based on adjustments of the iterative denoising process.  It gains unprecedented attention from both the research community and the public. Some of these methods use extra techniques to guide this process, such as CLIP guidance \cite{nichol2021glide,avrahami2022blended}, classifier\cite{dhariwal2021guided,zhao2022egsde} and low-pass filter\cite{choi2021ilvr,zhao2022egsde}. \cite{meng2021sdedit} uses a noised version of the input image as a starting point for the denoising process and pursues a good trade-off between realism and faithfulness of manipulated image. To strictly manipulate a specific region, \cite{avrahami2022blended} also uses the mask to blend input and denoised images during this process. All diffusion-based image editing approaches fall into the category that injecting guidance into the source image through the iterative process. They still follow a similar iterative routine to image generation. When performing editing, they require thousands of times forwarding.

%% redandant
 However, unlike the image generation process that ultimately creates an image from noise, image editing only involves several regional modifications or some specific attributes modification. \cite{} claims that different denoising steps take charge of manipulating different attributes. A straightforward hypothesis is that only some key steps contribute to our desired editing attributes, and it is redundant to maintain all the denoising steps in image editing. 

%% harmful
% Moreover, it is still an open problem \cite{choi2021ilvr,meng2021sdedit,avrahami2022blended} at which steps of the denoising process explicitly intervene in different attributes of manipulation. Different steps can lead to very different editing results. 
Moreover, involving guidance-irrelevant steps even modify some preserved properties, hence harming the consistency of our edited images with the source images. For example, when a step with heavy noise is sampled, the diffusion model is basically changing the low-frequency information, like building the coarse structure. It hasn't been aware of any fine-grained attributes. But if you still give a fine-grained guided direction in this step, the diffusion model will change the guidance-irrelevant attributes of the source image according to a misleading direction, like brightness and outlines. (shown in Fig. ~\ref{}) Consequently, the inconsistency appears in the source image.

%% so step choosing is essential in image editing, but the current framework is too rigid to do that.
However, the current image editing frameworks are too rigid to do this. Due to the iterative process, they have to sample the steps one by one in descending order. Even if we use the respacing strategy in the DDIM\cite{} to skip unwanted steps, we will still face the problem of image collapse when the sampled steps are few or the gap between two steps is significant. The inflexibility urges us to discover a more adaptable approach to remove the unwanted steps when using the diffusion model.
Based on the above hypothesis, we hope to find a way that excludes the harmful steps and merely uses the key steps during the iterative process, thus we can accelerate the editing process and maintain consistency with the source image. 

%% motivated by plug and play
Recently, \cite{graikos2022diffusion,poole2022dreamfusion} has demonstrated another paradigm using diffusion models as a plug-and-play prior. 
Using one independently trained diffusion model and arbitrary differentiable constraints on $\mathbf{x}$ given some additional information $\mathbf{y}$, one could use the gradient from the diffusion model to optimize $\mathbf{x}$, and thus achieve image generation given condition $\mathbf{y}$. 
If this constraint is deterministic, such as a latent variable model, we can use the gradient directly to optimize the latent variable $\mathbf{y}$. 
Also, it is possible to optimize the parameters of neural networks using differentiable image parameterization\cite{poole2022dreamfusion}. 
This technique motivates us to build a non-iterative diffusion-based image editing paradigm by using diffusion gradient priors as guidance. In this paper, we propose using a trained diffusion model as the image-level guidance rather than using it as the image synthesizer. When performing editing, only gradients will be applied to the source image. With this non-iterative manner, flexible sampling of denoising steps becomes available. 

%% t policy
In addition, this framework offers us an easier way to identify the desired steps by explicitly showing the diffusion gradient priors. We discover that the gradient information flows to the source image significantly indicates the importance of steps. According to this analysis, we introduce a combination of metrics including gradient entropy and absolute gradient value. Using these metrics, we design a step-searching algorithm to select appropriate steps to accelerate the editing process and enforce consistency with the source image.

%% summary
In summary, our contributions are three manifolds:
\begin{itemize}
  \item We propose an image manipulation framework using a multi-modal diffusion gradient as prior and implement a flexible non-iterative image editing paradigm.
  \item We introduce a search algorithm based on gradient-level metrics to find suitable time steps for an editing direction, which can improve the quality and efficiency of the editing.
  \item Our experiments demonstrate our method's effectiveness in both the qualitative and the quantitative aspects.
\end{itemize}


==> legacy/01_intro_v1.tex <==
\section{Introduction}
\label{sec:intro}
Diffusion models have achieved an overwhelming performance on the image generation task, and diffusion models conditioned on natural language text prompts\cite{saharia2022imagen, rombach2022stablediffusion, nichol2021glide, ramesh2022dalle2} have shown their ability of diverse and controllable image synthesis. 
The promising results further spur computer scientists to fully utilize the diffusion models in downstream applications, such as image manipulation.

Conventional methods that manipulate images with diffusion models  \cite{choi2021ilvr,meng2021sdedit,avrahami2022blended,zhao2022egsde,dhariwal2021guided} are based on the adjustments of the iterative denoise process. In each step of the process, additional guidance and techniques are introduced, such as CLIP\cite{nichol2021glide,avrahami2022blended}, classifier\cite{dhariwal2021guided,zhao2022egsde}, low-pass filter\cite{choi2021ilvr,zhao2022egsde}, mask\cite{avrahami2022blended}, etc. Thus they can finally achieve the image manipulations to the target semantics, such as human attribute translation and style modifications.
% summarize existing methods
All these methods follow a similar iterative routine to image generation. When performing editing, they require thousands of times forwarding from noise to an image.

% editing is not like generation, only changing specific property
However, unlike image generation, image editing only involves several regional modifications or some specific semantics modification.
% properties are related to different stages, coarse mid fine.
Also, different modifications of visual properties correspond to different stages of the diffusion generation process. For example, we can categorize the diffusion generation process into coarse, content, and clean-up stages\cite{choi2022perception}. When performing face expression manipulation, we only need to change the content.
% so ..., because other stages are redundant even harmful.
Therefore, it is intuitive(straightforward) to perform image editing merely at the guidance-related stages, since involving other stages is redundant and even harmful.
% some current methods notice this and use naive ways to improve
To avoid undesirable modifications, existing methods use auxiliary information\cite{avrahami2022blended} or heuristic steps skipping\cite{choi2021ilvr,zhao2022egsde, avrahami2022blended} as improvements.

% however, due to the inflexibility, still cannot accurately choose stages.
However, these improvements still cannot guarantee the accurate choice of stages. The fundamental reason is that the inference stage of image manipulation is a reverse diffusion process, so they can not perform manipulation with only a specific stage, such as the content stage. 
% we solve that
The inflexibility urges us to discover a more adaptable approach to removing unwanted steps using the diffusion model.

% the paper plug-and-play motivate us
% it is xx.(introduction)
Recent works have proven that diffusion models can also be used as a prior \cite{graikos2022diffusion,poole2022dreamfusion}. 
Combining independently trained diffusion models with arbitrary differentiable constraints on $\mathbf{x}$ given some additional information $\mathbf{y}$, we can optimize a random image with the training objective of the diffusion model to obtain a sample $\mathbf{x}$ from $p(x\mid y)$. 
Suppose this constraint is deterministic, such as $x=f(y)$, where $f()$ is a differentiable network, and we can obtain a sample from the diffusion model by indirectly optimizing the latent variable $\mathbf{y}$. 
For example, $y$ could be parameters of a network, and $f$ is the differentiable rendering process that transforms $y$ to synthesize sample $x$ of pre-trained diffusion models.
% it cannot do xxx.

% we modified it. the new framework is xxx. 
In this work, we novelly extend this paradigm to a new scenario. We define $f(\cdot)$ as an image manipulation network and optimize it with diffusion prior. 
It means we try to optimize a translation parameterized by a network with diffusion prior. After this translation, the input image $y$ will become a sample from the diffusion prior. Significantly when this diffusion is multi-modal, we can optimize a translation that guides images toward a mode defined by natural language prompts. 

% advantages1: flexible.
This paradigm benefits us from two perspectives. Firstly, it releases our dependency on the diffusion model process for image manipulation in the inference stage. In the training stage, we have the flexibility to choose diffusion steps that are useful for each manipulation. 
% advantages2: explicitly indicates the step's importance. callback一下open problem
Secondly, the gradient from the training losses acts as an explicit indication of image-edits direction, making it easier to identify the desired steps. We carefully design a combination of metrics, including gradient entropy and absolute gradient value to reflect the preference of steps. 
% adv1 and adv2 make solved xxx, making our work good.
Using these metrics, we create a step-searching algorithm to select appropriate steps to accelerate the editing process and enforce consistency with the source image.

% summary
In summary, our contributions are three manifolds:
\begin{itemize}
  \item We propose an image manipulation framework using a multi-modal diffusion gradient as prior and implement a flexible non-iterative image editing paradigm.
  \item We introduce a search algorithm based on gradient-level metrics to find suitable time steps for an editing direction, which can improve the quality and efficiency of the editing.
  \item Our experiments demonstrate our method's effectiveness in both the qualitative and the quantitative aspects.
\end{itemize}




==> legacy/01_intro_v10.tex <==
\section{Introduction}
\label{sec:intro}
% Diffusion models 
In recent years, diffusion model \cite{sohl2015deep,ho2020ddpm,song2020ddim,dhariwal2021guided,nichol2021glide,saharia2022imagen,ramesh2022dalle2,rombach2022stablediffusion,song2019score1,song2020score2} has attracted great attention in both academic and industrial communities. 
It models the Markov transition from a Gaussian distribution to a data distribution so that it can generate high-quality images in a sequential way. 
With the elegant formulation, it achieves state-of-the-art performance in various image generation benchmarks. Meanwhile, text-to-image diffusion models \cite{saharia2022imagen, rombach2022stablediffusion, nichol2021glide, ramesh2022dalle2} also demonstrate their impressive capacity in controllable image synthesis, enabling a wide range of practical applications. Among them, one of the most interesting applications is image manipulation. 

% Conventional methods that manipulate images with diffusion models 
In general, diffusion models manipulate images by injecting guidance information to each step of the inference process, where the guidance information could be generated from CLIP \cite{nichol2021glide,avrahami2022blended}, classifier \cite{dhariwal2021guided,zhao2022egsde}, low-pass filter \cite{choi2021ilvr,zhao2022egsde}, mask \cite{avrahami2022blended}, a reference image\cite{meng2021sdedit}, etc. 
Although effective, their editing speed is pretty slow, e.g., when choosing total step equals as 1000, it may take 18.3 minutes to edit a 1024 x 1024 image, regardless of how subtle the editing effect is. The reason is that to edit an image, these methods need to start from a Gaussian noise and inject the guidance information in every step throughout the generation process, which takes a lot of time. 
Some recent works \cite{avrahami2022blended,avrahami2022blendedlatent,meng2021sdedit,choi2021ilvr} observe that guidance only needs to be applied from an intermediate step to the final one.
This could marginally accelerate the editing process. Nevertheless, they still require a few steps to be involved, and thus, their inference time is still high. 


In this work, we take a different viewpoint to leverage a diffusion model for image manipulation.
Unlike existing methods \cite{nichol2021glide,avrahami2022blended,dhariwal2021guided,zhao2022egsde,choi2021ilvr} that directly manipulate images progressively with diffusion models, we train an efficient image manipulator under the guidance of diffusion models. 
Especially, we reuse the diffusion training loss to optimize the image manipulator network.
% 这种做法类似将diffusion model作为一种指导先验，为我们的image manipulator提供编辑的方向
Our approach uses the diffusion model to provide image-wise edits for our image manipulator. 
To implement different edits more easily and efficiently, we use text-to-image diffusion models.
After optimization, our image manipulator can edit an image with only a single forward step, and also possible to generalize to more images. Therefore, our framework avoids the expensive time consumption during inference while benefiting from the rich modes of the diffusion model.


\begin{figure}[htbp]
    \centering
    \includegraphics[width=.5\textwidth]{figs/t_observation.pdf}
    \caption{Various timesteps lead to various results}
    \label{t-observation}
\end{figure}

In addition, optimization with diffusion models requires a timestep as input and we observed that passing various timesteps leads to various editing results, as shown in Fig.\ref{t-observation}. The red boxes in this figure points out the best result. For different edit, different timesteps achieve the optimal result. 
% It indicates that choosing the proper timesteps in our framework is especially significant.
This indicates that the diffusion model is dealing with different semantic information at different steps. 
To find the semantic-related timestep for each edit, we need an effective metric. 
For one edit, we analyze the gradients that the diffusion model provides to the image at each step and propose a metric that mix the internal entropy and L1 norm of this gradient map together, namely the hybrid quality score. 
This metric is a good indicator of the quality of diffusion guidance, higher quality will help to edit more effectively.
Then, we propose a step-pruning strategy based on our hybrid quality score. 
This strategy helps us find the most critical timesteps, which not only improves our training efficiency but also improves the quality of image manipulation

In summary, our contributions are three manifolds:
\begin{itemize}
  \item We propose a novel image editing paradigm by passing diffusion gradient to another image manipulator network. This paradigm supports efficient and effective editing with only one forward step.
  \item With the help of our paradigm, we design the timestep selection strategy from the perspective of information entropy. Based on this, we can train our image editing network more efficiently.
  \item Our experiments demonstrate our method's effectiveness and efficiency in both the qualitative and the quantitative aspects.
\end{itemize}




==> legacy/01_intro_v11.tex <==
\section{Introduction}
\label{sec:intro}
% Diffusion models 
In recent years, diffusion model \cite{sohl2015deep,ho2020ddpm,song2020ddim,dhariwal2021guided,nichol2021glide,saharia2022imagen,ramesh2022dalle2,rombach2022stablediffusion,song2019score1,song2020score2} has attracted great attention in both academic and industrial communities. 
It models the Markov transition from a Gaussian distribution to a data distribution so that it can generate high-quality images in a sequential way. 
With the elegant formulation, it achieves state-of-the-art performance in various image generation benchmarks. Meanwhile, text-to-image diffusion models \cite{saharia2022imagen, rombach2022stablediffusion, nichol2021glide, ramesh2022dalle2} also demonstrate their impressive capacity in controllable image synthesis, enabling a wide range of practical applications. Among them, one of the most interesting applications is image manipulation. 

\begin{figure}[htbp]
    \centering
    \includegraphics[width=8cm]{figs/comparison.pdf}
    \caption{\textbf{Comparisons between diffusion-based image manipulation methods (a) and ours (b)}. With the idea of SDD, we can manipulate the image without progressive inference.}
    \label{comparison}
\end{figure}

% Conventional methods that manipulate images with diffusion models 
In general, diffusion models manipulate images by injecting guidance information to each timestep of the inference process, where the guidance information could be generated from CLIP \cite{nichol2021glide,avrahami2022blended}, classifier \cite{dhariwal2021guided,zhao2022egsde}, low-pass filter \cite{choi2021ilvr,zhao2022egsde}, mask \cite{avrahami2022blended}, a reference image\cite{meng2021sdedit}, etc. 
Although effective, their editing speed is pretty slow, e.g., when choosing total steps equal to 1000, it may take 93.3 seconds to edit a $1024\times 1024$ image, regardless of how subtle the editing effect is. The reason is that to edit an image, these methods need to start from a Gaussian noise and inject the guidance information in every timestep throughout the generation process, which takes a lot of time. 
Some recent works \cite{avrahami2022blended,avrahami2022blendedlatent,meng2021sdedit,choi2021ilvr} observe that guidance only needs to be applied from an intermediate step to the final one.
This could marginally accelerate the editing process. Nevertheless, they still require quite a few steps to be involved, and thus, their inference time is still high.


In this work, we take a different viewpoint to leverage a diffusion model for image manipulation.
As shown in Fig. \ref{comparison}, unlike existing methods \cite{nichol2021glide,avrahami2022blended,dhariwal2021guided,zhao2022egsde,choi2021ilvr} that directly manipulate images progressively with diffusion models, we train an efficient image manipulator supervised by a pretrained diffusion model, which largely accelerates the editing speed. Specifically, our model takes a feedforward model (e.g., latent space image manipulation model \cite{patashnik2021styleclip} or image-to-image translation model \cite{isola2017image}) as the manipulator, and a text-guided diffusion model (e.g., latent diffusion \cite{rombach2022stablediffusion}) as the teacher. During training, the manipulated image is diffused and fed to the teacher diffusion model, and the diffusion model would produce gradient supervision based on the text condition. In this sense, it is expected that the manipulator could mimic the promising generation capacity of the diffusion model.


It should be noted that turning this intuitive idea into practice is not trivial. Besides the noisy image and the text condition, the diffusion model also takes a timestep $t$ as input. And we find that different timesteps lead to very different results (will be shown in Fig. \ref{t-observation}).  
The reason could be that, for a diffusion model, different timesteps correspond to different levels of information, and thus the generated gradient is also different. Using inappropriate timesteps for supervision may lead to suboptimal results.  
To cope with this, we propose the hybrid quality score, an effective indicator that helps to filter out those inappropriate timesteps. 
This indicator is built upon the entropy and $L_1$ norm of the gradient from the diffusion model, and is shown to be highly correlated with the edit quality. As such, our model could avoid learning with improper steps. This is advantageous compared with existing works \cite{nichol2021glide,avrahami2022blended,dhariwal2021guided,zhao2022egsde,choi2021ilvr}, which do manipulation progressively and thus could inevitably be affected by the harmful timesteps. Extensive experiments demonstrate that our model achieves the state-of-the-art performance with much faster editing speed. 
Our contributions are summarized as follows:
\begin{itemize}
  \item We propose a novel image manipulation approach that takes a well-trained diffusion model as a teacher to train another image manipulation network. This largely improves the editing speed.  
  \item We discover that there exist some timesteps that could harm the performance, and propose a hybrid quality score to filter out them. This largely improves our generation's quality. 
  \item Our experiments demonstrate our method's effectiveness and efficiency in both the qualitative and the quantitative aspects.
\end{itemize}




==> legacy/01_intro_v12.tex <==
\section{Introduction}
\label{sec:intro}
% Diffusion models 
In recent years, diffusion model \cite{sohl2015deep,ho2020ddpm,song2020ddim,dhariwal2021guided,nichol2021glide,saharia2022imagen,ramesh2022dalle2,rombach2022stablediffusion,song2019score1,song2020score2} has attracted great attention in both academic and industrial communities. 
It models the Markov transition from a Gaussian distribution to a data distribution to generate high-quality images sequentially. 
The elegant formulation achieves state-of-the-art performance in various image generation benchmarks. Meanwhile, text-to-image diffusion models \cite{saharia2022imagen, rombach2022stablediffusion, nichol2021glide, ramesh2022dalle2} also demonstrate their impressive capacity in controllable image synthesis, enabling a wide range of practical applications. Among them, one of the most interesting applications is image manipulation. 

\begin{figure}[htbp]
    \centering
    \includegraphics[width=8cm]{figs/intro_tradeoff.pdf}
    \caption{\textbf{Editability and fidelity trade-off of diffusion-based image manipulation.} The leftmost is the input image. For each manipulation, we add increasing noise levels from left to right and then denoise the image. Different manipulations require different levels of noise for successful semantic manipulation.}
    \label{comparison}
\end{figure}

A typical text-guidance manipulation pipeline is to invert the input image to a noisy latent and then denoise this latent with a given text prompt. The inversion process can be the simple noise adding \cite{meng2021sdedit} or the DDIM inversion \cite{su2022dual, song2020ddim}. 
% 看图说话
% In the such a pipeline, we need to manually control the noisy level of the inverted latent, producing an editability-fidelity tradeoff problem. 
There is an editability-fidelity tradeoff in such pipelines, as shown in Fig.~\ref{fig:intro-pipeline}. 
% 解释trade-off
Adding a lot of noise to the original image gives the diffusion model more freedom to manipulate the image, but it also makes it harder to retain original semantics when denoising back, and vice versa. 

% 更深刻的说， 这种trade-off导致了一些编辑必定失败
More importantly, this trade-off can lead to some unsuccessful manipulations, such as ``white hair" in Fig.~\ref{fig:intro-pipeline}. This is because the diffusion model processes different semantics at different stages \cite{choi2022perception}.  If our manipulation corresponds to the semantics in the early stages, we have to add more noise, and hence losing nearly all information from the original image.
To overcome the failure caused by the trade-off, existing methods attempt to incorporate more guidance information, such as using masks to limit the manipulation region \cite{avrahami2022blended, avrahami2022blendedlatent, lugmayr2022repaint}. This is useful for local image manipulation, but for some global structures, such as changing the pose of a human face, it still fails to solve the problem.

In this work, we take a different viewpoint to leverage a diffusion model for image manipulation.
Unlike existing methods that directly manipulate images progressively with diffusion models, we train an efficient image manipulator supervised by a pretrained diffusion model. 
Specifically, our model takes a feedforward model (e.g., latent space image manipulation model \cite{patashnik2021styleclip} or image-to-image translation model \cite{isola2017image}) as the manipulator, and a text-guided diffusion model (e.g., latent diffusion \cite{rombach2022stablediffusion}) as the supervisor. During training, the manipulated image is diffused and fed to the diffusion model, and the diffusion model produces gradient supervision based on the text condition. In this sense, it is expected that the manipulator could mimic the promising generation capacity of the diffusion model.
% Specifically, our model takes a pre-trained feedforward model as the manipulator (e.g., the latent space image manipulation model \cite{patashnik2021styleclip} or the image-to-image translation model \cite{isola2017image}). And we take a text-guided diffusion model as the supervisor (e.g., latent diffusion \cite{rombach2022stablediffusion}). During training, the input image is fed to the manipulator. Then, the manipulated image is diffused and sent to the supervisor diffusion model. The diffusion model will produce gradient supervision based on the text condition. Finally, this supervision effects our manipulator through the back propagation. After the manipulator is trained, it is expected that the manipulator could mimic the promising generation capacity of the diffusion model. In this sense, we can impose regularization terms on the manipulator to ensure the fidelity. Therefore, we can combine the diffusion model's editability with the image manipulator's fidelity.

To learn such a manipulator, using correct semantic guidance is also crucial as shown in Fig. \ref{comparison} (b), only in the extra timestep can the diffusion model guide changing hair color. Other timesteps do not provide the semantic guidance needed for supervising the manipulator.
Therefore, we propose the hybrid quality score (HQS), an effective indicator that helps to filter out those inappropriate timesteps.
This indicator is built upon the entropy and $L_1$ norm of the gradient from the diffusion model and is shown to be highly correlated with the manipulation quality. As such, our model could avoid learning with improper timesteps. 

In addition to solving the trade-off problem of diffusion-based image manipulation, we have another benefit: our image manipulator requires only one forward for manipulation, and by learning in a specific domain, our image manipulator can manipulate images over the entire domain, which offsets the cost of training. Extensive experiments demonstrate the effectiveness of our methods.

Our contributions are summarized as follows:
\begin{itemize}
  \item We propose a novel image manipulation approach with a well-trained diffusion model to supervise another image manipulator. This avoids the trade-off problem of manipulating images with a diffusion process.
  \item We propose the hybrid quality score to detect semantic-related timesteps. Only during these timesteps can the diffusion model guide the image manipulator to perform accurate manipulations.
  \item Our experiments demonstrate our method's effectiveness and efficiency in both the qualitative and the quantitative aspects.
\end{itemize}





==> legacy/01_intro_v2.tex <==
\section{Introduction}
\label{sec:intro}
Diffusion models have achieved an overwhelming performance on the image generation task, and diffusion models conditioned on natural language text prompts\cite{saharia2022imagen, rombach2022stablediffusion, nichol2021glide, ramesh2022dalle2} have shown their ability of diverse and controllable image synthesis. 
The promising results further spur computer scientists to fully utilize the diffusion models in downstream applications, such as image manipulation.

Conventional methods that manipulate images with diffusion models  \cite{choi2021ilvr,meng2021sdedit,avrahami2022blended,zhao2022egsde,dhariwal2021guided} are based on the adjustments of the iterative denoise process. In each step of the process, additional guidance and techniques are introduced, such as CLIP\cite{nichol2021glide,avrahami2022blended}, classifier\cite{dhariwal2021guided,zhao2022egsde}, low-pass filter\cite{choi2021ilvr,zhao2022egsde}, mask\cite{avrahami2022blended}, etc. Thus they can finally achieve the image manipulations to the target semantics, such as human attribute translation and style modifications.
% summarize existing methods:并体现矛盾，即使小的局部修改需要这样整个迭代过程吗
All these methods follow a similar iterative routine to image generation. 
Even though editing only involves several regional modifications or some specific semantics modification, they still require the whole process from noise to an image. 

% 理论上，不同编辑使用迭代过程的对应阶段是一种更有效率的做法
Theoretically, in the editing task, it is more efficient to only use the corresponding stages of the generation process, because different stages are known to be responsible for different visual concepts \cite{choi2022perception}. 
For example, we only need to change the content when performing face expression manipulation.
% 更重要的是，整个迭代过程不仅多余还会有害
Moreover, involving other stages is redundant and even detrimental, as it may introduce some undesired modifications.

% 因此为了排除掉这些有害的步骤，这些方法不得不用一些navie的手段。缺点：他们并没有做到甄别
Because of this, existing methods fall short of consistent(accurate?) editing, so they have to resort to auxiliary information\cite{avrahami2022blended} or heuristic steps skipping\cite{choi2021ilvr,zhao2022egsde, avrahami2022blended} as improvements.
% 如何甄别编辑所对应的阶段以及如何只利用某一阶段变成了一个重要的问题
% We should identify the stage corresponding to each edit and use that stage exclusively for editing.
% problem1: 目前这些方法要么受限于灵活性
However, the inference of these methods depends on the generative process, and they can not perform manipulation with only a specific stage. 

% 我改成了下面
Therefore, existing methods have to resort to auxiliary information\cite{avrahami2022blended} or heuristic steps skipping\cite{choi2021ilvr,zhao2022egsde, avrahami2022blended} as improvements. But they still fall short of consistent(accurate?) editing. Due to their strong dependency on the iterative process, they can not perform manipulation with only a few selected steps. 
% problem2: 要么很难讨论该问题
Meanwhile, they lack an effective indicator to identify useful steps for editing.
% 所以我们不得不寻求新的手段来解决
These reasons urge us to discover a more adaptable approach to removing unwanted steps using the diffusion model.

% the paper plug-and-play motivate us
% it is xx.(introduction)
Recent works have proven that diffusion models can also be used as a prior \cite{graikos2022diffusion,poole2022dreamfusion}. 
Combining independently trained diffusion models with arbitrary differentiable constraints on $\mathbf{x}$ given some additional information $\mathbf{y}$, we can optimize a random image with the training objective of the diffusion model to obtain a sample $\mathbf{x}$ from $p(x\mid y)$. 
Suppose this constraint is deterministic, such as $x=f(y)$, where $f()$ is a differentiable network, and we can obtain a sample from the diffusion model by indirectly optimizing the latent variable $\mathbf{y}$. 
For example, $y$ could be parameters of a network, and $f$ is the differentiable rendering process that transforms $y$ to synthesize sample $x$ of pre-trained diffusion models.
% it cannot do xxx.

% we modified it. the new framework is xxx. 
In this work, we novelly extend this paradigm to a new scenario. We define $f(\cdot)$ as an image manipulation network and optimize it with diffusion prior. 
It means we try to optimize a translation parameterized by a network with diffusion prior. After this translation, the input image $y$ will become a sample from the diffusion prior. Significantly when this diffusion is multi-modal, we can optimize a translation that guides images toward a mode defined by natural language prompts. 

% advantages1: flexible.
This paradigm benefits us from two perspectives. Firstly, it releases our dependency on the diffusion model process for image manipulation in the inference stage. In the training stage, we have the flexibility to choose diffusion steps that are useful for each manipulation. 
% advantages2: explicitly indicates the step's importance. callback一下open problem
Secondly, the gradient from the training losses acts as an explicit indication of image-edits direction, making it easier to identify the desired steps. We carefully design a combination of metrics, including gradient entropy and absolute gradient value to reflect the preference of steps. 
% adv1 and adv2 make solved xxx, making our work good.
Using these metrics, we create a step-searching algorithm to select appropriate steps to accelerate the editing process and enforce consistency with the source image.

% summary
In summary, our contributions are three manifolds:
\begin{itemize}
  \item We propose an image manipulation framework using a multi-modal diffusion gradient as prior and implement a flexible non-iterative image editing paradigm.
  \item We introduce a search algorithm based on gradient-level metrics to find suitable time steps for an editing direction, which can improve the quality and efficiency of the editing.
  \item Our experiments demonstrate our method's effectiveness in both the qualitative and the quantitative aspects.
\end{itemize}




==> legacy/01_intro_v3.tex <==
\section{Introduction}
\label{sec:intro}
Diffusion models have achieved an overwhelming performance on the image generation task, and diffusion models conditioned on natural language text prompts\cite{saharia2022imagen, rombach2022stablediffusion, nichol2021glide, ramesh2022dalle2} have shown their ability of diverse and controllable image synthesis. 
The promising results further spur computer scientists to fully utilize the diffusion models in downstream applications, such as image manipulation.

Conventional methods that manipulate images with diffusion models  \cite{choi2021ilvr,meng2021sdedit,avrahami2022blended,zhao2022egsde,dhariwal2021guided} are based on the adjustments of the iterative denoise process. In each step of the process, additional guidance and techniques are introduced, such as CLIP\cite{nichol2021glide,avrahami2022blended}, classifier\cite{dhariwal2021guided,zhao2022egsde}, low-pass filter\cite{choi2021ilvr,zhao2022egsde}, mask\cite{avrahami2022blended}, etc. Thus they can finally achieve the image manipulations to the target semantics, such as human attribute translation and style modifications.
% summarize existing methods:并体现矛盾，即使小的局部修改需要这样整个迭代过程吗
All these methods follow a similar iterative routine to image generation. 
Even though editing only involves several regional modifications or some specific semantics modification, they still require the whole process from noise to an image. 

% 理论上，不同编辑使用迭代过程的对应阶段是一种更有效率的做法
Existing theories have demonstrated that different stages are responsible for different visual concepts \cite{choi2022perception}. Therefore, in the editing task, it is more efficient to only use the editing-related(corresponding) stages of the generation process. 
For example, when manipulating the facial expression, we only need to employ the content stage.
% 更重要的是，整个迭代过程不仅多余还会有害
Moreover, involving other stages is redundant and even detrimental, as it may introduce some undesired modifications.
 
Therefore, existing methods have to resort to auxiliary information\cite{avrahami2022blended} or heuristic steps skipping\cite{choi2021ilvr,zhao2022egsde, avrahami2022blended} as improvements, but they still fall short of consistent editing.
% problem1: 灵活性不够
1) Due to their strong dependency on the iterative process, they can not perform manipulation with only a few selected steps. 
% problem2: 要么很难讨论该问题
2) Meanwhile, they lack an effective indicator to identify useful steps for editing.
% 所以我们不得不寻求新的手段来解决
These reasons urge us to discover a more adaptable approach to removing unwanted steps using the diffusion model.


Recent works leverage the structure of diffusion models to enable tractable sampling via optimization — a loss function that, when minimized, yields a sample in pixel space\cite{graikos2022diffusion}.
Motivated by this work, we propose a novel image-editing paradigm that solved the inflexibility problem. 
Firstly, we theoretically extend their optimization strategy from image generation to image editing. 
% 详细介绍我们的方法流程
% ...
Secondly, we introduce a more proper optimization target rather than directly optimizing the pixels, since the latter often falls into the low fidelity problem\cite{graikos2022diffusion}. 
Significantly, when this diffusion model is multi-modal, we can obtain a translation that guides images toward a mode defined by natural language prompts.
The most remarkable advantage of the proposed method is the flexibility of step selection. 
% By using the diffusion model as optimization priors, we implement a non-iterative editing framework. as 
% 很想补一句 生怕听不懂
We can just sample whatever stages you want.

% 放到method?
% this loss function on the parameters of the image editing network, rather than directly optimizing the pixels, since the latter often falls into the low fidelity problem\cite{graikos2022diffusion}. 

In addition to the flexibility of step selection, our method also explicitly shows the gradient from the training losses. Furthermore, the gradient can be used as an indication of image-edits direction, making it easier to identify the desired steps. We carefully design a combination of metrics, including gradient entropy and absolute gradient value, to reflect the preference of steps. 
Using these metrics, we create a step-searching algorithm to select appropriate steps to accelerate the editing process and enforce consistency with the source image.

% 这里我们可以把denoise过程变成optimization过程，因此可以更灵活的选取t了

% However, 直接搬到editing 有问题
% However, even in image generation tasks, sampling pixels with this method does not guarantee the fidelity of results, and some post-processing is required \cite{graikos2022diffusion}. 

% 3D那边去
Instead of sampling pixels, we can also sample parameters of a 3D volume so that its rendered pixels look like a sample from the frozen diffusion models \cite{poole2022dreamfusion}. 
Even without further discussion of stages, it can perform good results in image generation tasks.


% % advantages1: flexible.
% This paradigm benefits us from two perspectives. Firstly, it releases our dependency on the diffusion model process for image manipulation in the inference stage. In the training stage, we have the flexibility to choose diffusion steps that are useful for each manipulation. 
% % advantages2: explicitly indicates the step's importance. callback一下open problem
% Secondly, the gradient from the training losses is an explicit indication of image-edits direction, making it easier to identify the desired steps. We carefully design a combination of metrics, including gradient entropy and absolute gradient value, to reflect the preference of steps. 
% % adv1 and adv2 make solved xxx, making our work good.

% summary
In summary, our contributions are three manifolds:
\begin{itemize}
  \item We propose an image manipulation framework using a multi-modal diffusion gradient as prior and implement a flexible non-iterative image editing paradigm.
  \item We introduce a search algorithm based on gradient-level metrics to find suitable time steps for an editing direction, which can improve the quality and efficiency of the editing.
  \item Our experiments demonstrate our method's effectiveness in both the qualitative and the quantitative aspects.
\end{itemize}




==> legacy/01_intro_v4.tex <==
\section{Introduction}
\label{sec:intro}
Diffusion models\cite{sohl2015deep,ho2020ddpm,song2020ddim,dhariwal2021guided,nichol2021glide,saharia2022imagen,ramesh2022dalle2,rombach2022stablediffusion,song2019score1,song2020score2} have achieved an overwhelming performance on the image generation task, and diffusion models conditioned on natural language text prompts\cite{saharia2022imagen, rombach2022stablediffusion, nichol2021glide, ramesh2022dalle2} have shown their ability of diverse and controllable image synthesis. 
The promising results further spur computer scientists to fully utilize the diffusion models in downstream applications, such as image editing.

Conventional methods that manipulate images with diffusion models  \cite{choi2021ilvr,meng2021sdedit,avrahami2022blended,zhao2022egsde,dhariwal2021guided} are based on the adjustments of the iterative denoise process. In each step of the process, additional guidance and techniques are introduced, such as CLIP\cite{nichol2021glide,avrahami2022blended}, classifier\cite{dhariwal2021guided,zhao2022egsde}, low-pass filter\cite{choi2021ilvr,zhao2022egsde}, mask\cite{avrahami2022blended}, etc. Thus they can finally achieve the image editings to the target semantics, such as human attribute translation and style modifications.
% summarize existing methods:并体现矛盾，即使小的局部修改需要这样整个迭代过程吗
All these methods follow a similar iterative routine to image generation. 
Even though editing only involves several regional modifications or some specific semantics modification, they still require the whole process from noise to an image. 

% 理论上，不同编辑使用迭代过程的对应阶段是一种更有效率的做法
Existing theories have demonstrated that different stages are responsible for different visual concepts \cite{choi2022perception}. Therefore, it is more efficient to use the editing-related(corresponding) stages of the generation process in the editing task. 
For example, we only need to employ the content stage when manipulating the facial expression.
% 更重要的是，整个迭代过程不仅多余还会有害
Moreover, involving other stages is redundant and even detrimental, as it may introduce some undesired modifications.
 
Therefore, existing methods have to resort to auxiliary information\cite{avrahami2022blended} or heuristic steps skipping\cite{choi2021ilvr,zhao2022egsde, avrahami2022blended} as improvements, but they still fall short of consistent editing.
% problem1: 灵活性不够
1) Due to their strong dependency on the iterative process, they can not perform editing with only a few selected steps. 
% problem2: 很难讨论该问题
2) They lack an effective indicator to identify useful steps for editing.
% 所以我们不得不寻求新的手段来解决
These reasons urge us to discover a more adaptable approach to removing unwanted steps using the diffusion model.

% 可以选t
Recent work demonstrates that we can leverage the training process of diffusion models to generate images \cite{graikos2022diffusion}. 
This method computes the training loss of diffusion models in arbitrary time steps and backpropagates the gradient to optimize an image.
Motivated by this work, we propose a novel image-editing paradigm that utilizes this optimization strategy to support step selection.
Secondly, we introduce a more appropriate and advanced optimization target rather than directly optimizing the pixels since the latter often falls into the low fidelity problem\cite{graikos2022diffusion} - 
Given an output image from an arbitrary image editing network, we compute the diffusion training loss and backpropagate its gradient to the image editing network. 
Another advantage of optimizing the parameters is that we can complete the editing of the image with one forward.
Significantly, when this diffusion model is multi-modal, we can obtain a network that guides images toward a mode defined by natural language prompts. 

% 怎么选t
In addition to the flexibility of step selection, we observed that information carried by loss gradient greatly facilitates us to analyze the relationship between different steps and different editings. Considering that the diffusion generation process is a disorder-to-order entropy reduction process, we analyze the gradient from the perspective of entropy and empirically observe that it is a valuable indicator in step selection. Therefore, we propose a step-pruning strategy based on the entropy of the gradient. This strategy makes our method less susceptible to useless steps and can perform effective and efficient editing using diffusion knowledge.

% summary
In summary, our contributions are three manifolds:
\begin{itemize}
  \item We propose a novel image editing paradigm using diffusion knowledge, which supports efficient and effective editing with only one forward.
  \item We promote the discussion of the relationship between the diffusion process and the visual concept from the perspective of information entropy. Based on this, we propose a pruning strategy to train our image editing network more efficiently.
  \item Our experiments demonstrate our method's effectiveness in both the qualitative and the quantitative aspects.
\end{itemize}




==> legacy/01_intro_v5.tex <==
\section{Introduction}
\label{sec:intro}
Diffusion models\cite{sohl2015deep,ho2020ddpm,song2020ddim,dhariwal2021guided,nichol2021glide,saharia2022imagen,ramesh2022dalle2,rombach2022stablediffusion,song2019score1,song2020score2} have achieved an overwhelming performance on the image generation task, and diffusion models conditioned on natural language text prompts\cite{saharia2022imagen, rombach2022stablediffusion, nichol2021glide, ramesh2022dalle2} have shown their ability of diverse and controllable image synthesis. 
The promising results further spur computer scientists to fully utilize the diffusion models in downstream applications, such as image editing.

Conventional methods that manipulate images with diffusion models  \cite{choi2021ilvr,meng2021sdedit,avrahami2022blended,zhao2022egsde,dhariwal2021guided} are based on the adjustments of the iterative denoise process. In each step of the process, additional guidance and techniques are introduced, such as CLIP\cite{nichol2021glide,avrahami2022blended}, classifier\cite{dhariwal2021guided,zhao2022egsde}, low-pass filter\cite{choi2021ilvr,zhao2022egsde}, mask\cite{avrahami2022blended}, etc. Thus they can finally achieve the image editings to the target semantics, such as human attribute translation and style modifications.
% summarize existing methods:并体现矛盾，即使小的局部修改需要这样整个迭代过程吗
All these methods follow a similar iterative routine to image generation. 
Even though editing only involves several regional modifications or some specific semantics modification, they still require the whole process from noise to an image. 

% 理论上，不同编辑使用迭代过程的对应阶段是一种更有效率的做法
Existing theories have demonstrated that different stages are responsible for different visual concepts \cite{choi2022perception}. Therefore, it is more efficient to use the editing-related(corresponding) stages of the generation process in the editing task. 
For example, we only need to employ the content stage when manipulating the facial expression.
% 更重要的是，整个迭代过程不仅多余还会有害
Moreover, involving other stages is redundant and even detrimental, as it may introduce some undesired modifications.
 
Therefore, existing methods have to resort to auxiliary information\cite{avrahami2022blended} or heuristic steps skipping\cite{choi2021ilvr,zhao2022egsde, avrahami2022blended} as improvements, but they still fall short of consistent editing.
% problem1: 灵活性不够
1) Due to their strong dependency on the iterative process, they can not perform editing with only a few selected steps. 
% problem2: 很难讨论该问题
2) They lack an effective indicator to identify useful steps for editing.
% 所以我们不得不寻求新的手段来解决
These reasons urge us to discover a more adaptable approach to removing unwanted steps using the diffusion model.

% 可以选t
% in this work, we propose xxx that can adaptively select key steps in 
Recent work demonstrates that we can leverage the training process of diffusion models to generate images \cite{graikos2022diffusion}. 
This method computes the training loss of diffusion models in arbitrary time steps and backpropagates the gradient to optimize an image.
Motivated by this work, we propose a novel image-editing paradigm that utilizes this optimization strategy to support step selection.
Secondly, we introduce a more appropriate and advanced optimization target rather than directly optimizing the pixels since the latter often falls into the low fidelity problem\cite{graikos2022diffusion} - 
Given an output image from an arbitrary image editing network, we compute the diffusion training loss and backpropagate its gradient to the image editing network. 
Another advantage of optimizing the parameters is that we can complete the editing of the image with one forward.
Significantly, when this diffusion model is multi-modal, we can obtain a network that guides images toward a mode defined by natural language prompts. 

% 怎么选t
In addition to the flexibility of step selection, we observed that information carried by loss gradient greatly facilitates us to analyze the relationship between different steps and different editings. 
First, we convert the value of the gradient into confidence and then calculate the entropy of the confidence map. The lower the value, the more orderly the image-wise edit given by the diffusion model.
Therefore, we propose a step-pruning strategy based on the entropy of the confidence map. 
This strategy makes our method less susceptible to useless steps and can perform effective and efficient editing using diffusion knowledge.

% summary
In summary, our contributions are three manifolds:
\begin{itemize}
  \item We propose a novel image editing paradigm using diffusion knowledge, which supports efficient and effective editing with only one forward.
  \item We promote the discussion of the relationship between the diffusion process and the visual concept from the perspective of information entropy. Based on this, we propose a pruning strategy to train our image editing network more efficiently.
  \item Our experiments demonstrate our method's effectiveness in both the qualitative and the quantitative aspects.
\end{itemize}




==> legacy/01_intro_v6.tex <==
\section{Introduction}
\label{sec:intro}
Diffusion models\cite{sohl2015deep,ho2020ddpm,song2020ddim,dhariwal2021guided,nichol2021glide,saharia2022imagen,ramesh2022dalle2,rombach2022stablediffusion,song2019score1,song2020score2} have achieved an overwhelming performance on the image generation task, and diffusion models conditioned on natural language text prompts\cite{saharia2022imagen, rombach2022stablediffusion, nichol2021glide, ramesh2022dalle2} have shown their ability of diverse and controllable image synthesis. 
The promising results further spur computer scientists to fully utilize the diffusion models in downstream applications, such as image editing.

Conventional methods that manipulate images with diffusion models  \cite{choi2021ilvr,meng2021sdedit,avrahami2022blended,zhao2022egsde,dhariwal2021guided} are based on the adjustments of the iterative denoise process. In each step of the process, additional guidance and techniques are introduced, such as CLIP\cite{nichol2021glide,avrahami2022blended}, classifier\cite{dhariwal2021guided,zhao2022egsde}, low-pass filter\cite{choi2021ilvr,zhao2022egsde}, mask\cite{avrahami2022blended}, etc. Thus they can finally achieve the image editings to the target semantics, such as human attribute translation and style modifications.
% summarize existing methods:并体现矛盾，即使小的局部修改需要这样整个迭代过程吗
All these methods follow a similar iterative routine to image generation. 
Even though editing only involves fine-grained modifications, they still require the whole process from noise to an image. 

% 理论上，不同编辑使用迭代过程的对应阶段是一种更有效率的做法
Existing theories have demonstrated that different stages are responsible for different visual concepts in the diffusion denoising procrss\cite{choi2022perception}. Therefore, it is more efficient to merely use the editing-related stages of the generation process in the editing task. 
For example, we only need to employ the content stage when manipulating the facial expression.
% 更重要的是，整个迭代过程不仅多余还会有害
Moreover, involving other stages is redundant and even detrimental, as it may introduce some undesired modifications.
 
% Therefore, existing methods either mask modifications outside the region of interest in each step \cite{avrahami2022blended} or skip some of the harmful steps only at the beginning, 
% but they still fall short of consistent editing.
To avoid this problem, existing methods skip some of the harmful steps at the beginning based on their empirical observation\cite{avrahami2022blended, meng2021sdedit,choi2021ilvr}, but they still fall short of efficient editing. 
We attribute this problem to their strong dependency on the forward process. It is not feasible for them to select steps flexibly and use them in editing.
In addition, choosing steps is also very important, and they lack relevant analysis.
These reasons urge us to discover a more adaptable approach to removing unwanted steps using the diffusion model.

In this work, we propose a novel image editing paradigm with diffusion models that can adaptively select key steps for each editing.
Instead of progressively denoising the image like a diffusion model, our method takes pre-trained diffusion models a prior \cite{graikos2022diffusion}. 
This paradigm gives us the flexibility to select key steps.
Concretely, given an output image from an arbitrary image editing network, we compute the diffusion training loss at key steps and backpropagate its gradient to the image editing network. 
Significantly, when this pre-trained diffusion model is multi-modal, we can obtain a network that edits images with natural language prompts. 


In addition to the flexibility of step selection, we observed that the diffusion gradient information of images can greatly facilitate us to analyze the relationship between different steps and different editings. 
We convert the value of the gradient into confidence and then calculate the entropy of the confidence map. 
The lower the value, the more orderly the diffusion model gives the image-wise edit.
Therefore, we propose a step-pruning strategy based on the entropy of the gradient confidence map. 
This strategy makes our method less susceptible to useless steps and can perform effective and efficient editing using diffusion knowledge.

% summary
In summary, our contributions are three manifolds:
\begin{itemize}
  \item We propose a novel image editing paradigm by using diffusion knowledge as priors, which supports efficient and effective editing with only one forward.
  \item We promote the discussion of the relationship between the diffusion process and the visual concept from the perspective of information entropy. Based on this, we propose a pruning strategy to train our image editing network more efficiently.
  \item Our experiments demonstrate our method's effectiveness in both the qualitative and the quantitative aspects.
\end{itemize}




==> legacy/01_intro_v7.tex <==
\section{Introduction}
\label{sec:intro}
% Diffusion models \cite{sohl2015deep,ho2020ddpm,song2020ddim,dhariwal2021guided,nichol2021glide,saharia2022imagen,ramesh2022dalle2,rombach2022stablediffusion,song2019score1,song2020score2} have achieved an overwhelming performance on the image generation task, and diffusion models conditioned on natural language text prompts \cite{saharia2022imagen, rombach2022stablediffusion, nichol2021glide, ramesh2022dalle2} have shown their ability of diverse and controllable image synthesis. The promising results further spur researchers to fully utilize the diffusion models in downstream applications, such as image editing.
In recent years, diffusion model \cite{sohl2015deep,ho2020ddpm,song2020ddim,dhariwal2021guided,nichol2021glide,saharia2022imagen,ramesh2022dalle2,rombach2022stablediffusion,song2019score1,song2020score2} has attracted great attention in both academic and industrial communities. 
It models the Markov transition from a Gaussian distribution to the data distribution, so that it can generate high quality images in a sequential way. 
With the elegant formulation, it achieves the state-of-the-art performance in various image generation benchmarks. Meanwhile, conditional diffusion models \cite{saharia2022imagen, rombach2022stablediffusion, nichol2021glide, ramesh2022dalle2} also demonstrate their impressive capacity in controllable image synthesis, enabling a wide range of practical applications. Among them, one of the most interesting application is image manipulation. 

% Conventional methods that manipulate images with diffusion models \cite{choi2021ilvr,meng2021sdedit,avrahami2022blended,zhao2022egsde,dhariwal2021guided} are based on the adjustments of the iterative denoise process. In each step of the process, additional guidance and techniques are introduced, such as CLIP \cite{nichol2021glide,avrahami2022blended}, classifier \cite{dhariwal2021guided,zhao2022egsde}, low-pass filter \cite{choi2021ilvr,zhao2022egsde}, mask \cite{avrahami2022blended}, etc. Thus they can finally achieve the image editings to the target semantics, such as human attribute translation and style modifications.
% % summarize existing methods:并体现矛盾，即使小的局部修改需要这样整个迭代过程吗
% All these methods follow a similar iterative routine to image generation. Even though editing only involves fine-grained modifications, they still require the whole process from noise to an image.
In general, conditional diffusion models manipulate images by injecting guidance information to each step of the inference process, where the guidance information could be generated from CLIP \cite{nichol2021glide,avrahami2022blended}, classifier \cite{dhariwal2021guided,zhao2022egsde}, low-pass filter \cite{choi2021ilvr,zhao2022egsde}, mask \cite{avrahami2022blended}, etc. Although effective, these methods' editing speed is pretty slow, e.g., it takes xx minutes to edit a 1024 x 1024 image, regardless how subtle the editing effect could be. The reason is that, to edit an image, these methods need to start from a Guassian noise and inject the guidance information in every step throughout the generation process, which takes a lot of time. 
Some recent works \cite{avrahami2022blended,meng2021sdedit,choi2021ilvr} propose to impose guidance only in some relevant steps. 
This could marginally accelerate the editing process and improves the quality. Nevertheless, there are still quite a few steps need to be invloved, and thus the inference time assumption is still significant. 
% 另外，这些方法： 速度和 quality 有 trade-off

% % 理论上，不同编辑使用迭代过程的对应阶段是一种更有效率的做法
% Existing theories have demonstrated that different stages are responsible for different visual concepts in the diffusion denoising procrss\cite{choi2022perception}. Therefore, it is more efficient to merely use the editing-related stages of the generation process in the editing task. 
% For example, we only need to employ the content stage when manipulating the facial expression.
% % 更重要的是，整个迭代过程不仅多余还会有害
% Moreover, involving other stages is redundant and even detrimental, as it may introduce some undesired modifications.
 
% Therefore, existing methods either mask modifications outside the region of interest in each step \cite{avrahami2022blended} or skip some of the harmful steps only at the beginning, 
% but they still fall short of consistent editing.
% To avoid this problem, existing methods skip some of the harmful steps at the beginning based on their empirical observation \cite{avrahami2022blended, meng2021sdedit,choi2021ilvr}, but they still fall short of efficient editing. 
% We attribute this problem to their strong dependency on the forward process. It is not feasible for them to select steps flexibly and use them in editing.
% In addition, choosing steps is also very important, and they lack relevant analysis.
% These reasons urge us to discover a more adaptable approach to removing unwanted steps using the diffusion model.

% In this work, we propose a novel image editing paradigm with diffusion models that can adaptively select key steps for each editing.
% Instead of progressively denoising the image like a diffusion model, our method takes pre-trained diffusion models a prior \cite{graikos2022diffusion}. 
% This paradigm gives us the flexibility to select key steps.
In this work, we take a different viewpoint to leverage diffusion model for image manipulation.
Unlike existing methods \cite{nichol2021glide,avrahami2022blended,dhariwal2021guided,zhao2022egsde,choi2021ilvr} that directly manipulate images progressively with diffusion models, we train an efficient image manipulator under the guidance of diffusion models. Therefore, our framework benefits from the remarkable generation quality of diffusion model, while avoids its expensive time consumption during inference. 
Given an output image from an arbitrary image editing network, we compute the diffusion training loss at key steps and backpropagate its gradient to the image editing network. 
% Significantly, when this pre-trained diffusion model is multi-modal, we can obtain a network that edits images with natural language prompts. 
% 解释general idea， guidance of diffusion models，只需要说到 diffusion model provide gradient。

% diffusion model provide gradient 是没那么 simple的，不同的 t 出来的 graident 很不一样。用错 t 的话不work。我们observe了什么 ，based on this observation，propose了选t方法。
In addition to the flexibility of step selection, we observed that the diffusion gradient information of images can greatly facilitate us to analyze the relationship between different steps and different editings. 
We convert the value of the gradient into confidence and then calculate the entropy of the confidence map. 
The lower the value, the more orderly the diffusion model gives the image-wise edit.
Therefore, we propose a step-pruning strategy based on the entropy of the gradient confidence map. 
This strategy makes our method less susceptible to useless steps and can perform effective and efficient editing using diffusion knowledge.
% 你的 advantage 可以任意挑 t 。你 break 了 trade-off

% summary
In summary, our contributions are three manifolds:
\begin{itemize}
  \item We propose a novel image editing paradigm by using diffusion knowledge as priors, which supports efficient and effective editing with only one forward.
  \item We promote the discussion of the relationship between the diffusion process and the visual concept from the perspective of information entropy. Based on this, we propose a pruning strategy to train our image editing network more efficiently.
  \item Our experiments demonstrate our method's effectiveness in both the qualitative and the quantitative aspects.
\end{itemize}




==> legacy/01_intro_v8.tex <==
\section{Introduction}
\label{sec:intro}
% Diffusion models \cite{sohl2015deep,ho2020ddpm,song2020ddim,dhariwal2021guided,nichol2021glide,saharia2022imagen,ramesh2022dalle2,rombach2022stablediffusion,song2019score1,song2020score2} have achieved an overwhelming performance on the image generation task, and diffusion models conditioned on natural language text prompts \cite{saharia2022imagen, rombach2022stablediffusion, nichol2021glide, ramesh2022dalle2} have shown their ability of diverse and controllable image synthesis. The promising results further spur researchers to fully utilize the diffusion models in downstream applications, such as image editing.
In recent years, diffusion model \cite{sohl2015deep,ho2020ddpm,song2020ddim,dhariwal2021guided,nichol2021glide,saharia2022imagen,ramesh2022dalle2,rombach2022stablediffusion,song2019score1,song2020score2} has attracted great attention in both academic and industrial communities. 
It models the Markov transition from a Gaussian distribution to a data distribution so that it can generate high-quality images in a sequential way. 
With the elegant formulation, it achieves state-of-the-art performance in various image generation benchmarks. Meanwhile, conditional diffusion models \cite{saharia2022imagen, rombach2022stablediffusion, nichol2021glide, ramesh2022dalle2} also demonstrate their impressive capacity in controllable image synthesis, enabling a wide range of practical applications. Among them, one of the most interesting applications is image manipulation. 

% Conventional methods that manipulate images with diffusion models \cite{choi2021ilvr,meng2021sdedit,avrahami2022blended,zhao2022egsde,dhariwal2021guided} are based on the adjustments of the iterative denoise process. In each step of the process, additional guidance and techniques are introduced, such as CLIP \cite{nichol2021glide,avrahami2022blended}, classifier \cite{dhariwal2021guided,zhao2022egsde}, low-pass filter \cite{choi2021ilvr,zhao2022egsde}, mask \cite{avrahami2022blended}, etc. Thus they can finally achieve the image editings to the target semantics, such as human attribute translation and style modifications.
% % summarize existing methods:并体现矛盾，即使小的局部修改需要这样整个迭代过程吗
% All these methods follow a similar iterative routine to image generation. Even though editing only involves fine-grained modifications, they still require the whole process from noise to an image.
In general, conditional diffusion models manipulate images by injecting guidance information to each step of the inference process, where the guidance information could be generated from CLIP \cite{nichol2021glide,avrahami2022blended}, classifier \cite{dhariwal2021guided,zhao2022egsde}, low-pass filter \cite{choi2021ilvr,zhao2022egsde}, mask \cite{avrahami2022blended}, etc. 
Although effective, these methods' editing speed is pretty slow, e.g., it takes xx minutes to edit a 1024 x 1024 image, regardless of how subtle the editing effect could be. The reason is that, to edit an image, these methods need to start from a Gaussian noise and inject the guidance information in every step throughout the generation process, which takes a lot of time. 
Some recent works \cite{avrahami2022blended,meng2021sdedit,choi2021ilvr} propose to impose guidance only in some relevant steps. 
This could marginally accelerate the editing process. Nevertheless, they still require quite a few steps to be involved, and thus the inference time assumption is still high. 

% This paradigm gives us the flexibility to select key steps.
In this work, we take a different viewpoint to leverage a conditional diffusion model for image manipulation.
Unlike existing methods \cite{nichol2021glide,avrahami2022blended,dhariwal2021guided,zhao2022egsde,choi2021ilvr} that directly manipulate images progressively with diffusion models, we train an efficient image manipulator under the guidance of diffusion models. 
Given an output image from an arbitrary image manipulator network, we compute the diffusion training loss at key steps and backpropagate its gradient to the image manipulator network. After several iterations of optimizing, we finally obtain an image manipulator that can edit an image with only a single forward step. Therefore, our framework avoids the expensive time consumption during inference, while benefiting from the remarkable generation quality of the diffusion model.
In summary, our key idea is that we take a conditional diffusion model as guidance rather than the image manipulator.


In addition, we observe that passing various timesteps to the diffusion model leads to various editing results, as shown in Fig.\ref{}. It indicates that choosing the proper timesteps in our framework is especially significant.  
Fortunately, our framework offers us an explicit indicator of the important timesteps. The diffusion gradient flowing to edited images can greatly facilitate us to analyze which timesteps are needed. 
We convert the value of the gradient into confidence and then calculate the entropy of the confidence map. 
The lower the value, the more orderly the diffusion model gives the image-wise edit.
Therefore, we propose a step-pruning strategy based on the entropy of the gradient confidence map. 
This strategy makes our method less susceptible to useless steps and can perform effective and efficient editing using diffusion knowledge.

% summary
In summary, our contributions are three manifolds:
\begin{itemize}
  \item We propose a novel image editing paradigm by passing diffusion gradient to another image manipulator network. This paradigm supports efficient and effective editing with only one forward step.
  \item With the help of our paradigm, we design the timestep selection strategy from the perspective of information entropy. Based on this, we are able to train our image editing network more efficiently.
  \item Our experiments demonstrate our method's effectiveness and efficiency in both the qualitative and the quantitative aspects.
\end{itemize}




==> legacy/01_intro_v9.tex <==
\section{Introduction}
\label{sec:intro}
% Diffusion models \cite{sohl2015deep,ho2020ddpm,song2020ddim,dhariwal2021guided,nichol2021glide,saharia2022imagen,ramesh2022dalle2,rombach2022stablediffusion,song2019score1,song2020score2} have achieved an overwhelming performance on the image generation task, and diffusion models conditioned on natural language text prompts \cite{saharia2022imagen, rombach2022stablediffusion, nichol2021glide, ramesh2022dalle2} have shown their ability of diverse and controllable image synthesis. The promising results further spur researchers to fully utilize the diffusion models in downstream applications, such as image editing.
In recent years, diffusion model \cite{sohl2015deep,ho2020ddpm,song2020ddim,dhariwal2021guided,nichol2021glide,saharia2022imagen,ramesh2022dalle2,rombach2022stablediffusion,song2019score1,song2020score2} has attracted great attention in both academic and industrial communities. 
It models the Markov transition from a Gaussian distribution to a data distribution so that it can generate high-quality images in a sequential way. 
With the elegant formulation, it achieves state-of-the-art performance in various image generation benchmarks. Meanwhile, conditional diffusion models \cite{saharia2022imagen, rombach2022stablediffusion, nichol2021glide, ramesh2022dalle2} also demonstrate their impressive capacity in controllable image synthesis, enabling a wide range of practical applications. Among them, one of the most interesting applications is image manipulation. 

% Conventional methods that manipulate images with diffusion models \cite{choi2021ilvr,meng2021sdedit,avrahami2022blended,zhao2022egsde,dhariwal2021guided} are based on the adjustments of the iterative denoise process. In each step of the process, additional guidance and techniques are introduced, such as CLIP \cite{nichol2021glide,avrahami2022blended}, classifier \cite{dhariwal2021guided,zhao2022egsde}, low-pass filter \cite{choi2021ilvr,zhao2022egsde}, mask \cite{avrahami2022blended}, etc. Thus they can finally achieve the image editings to the target semantics, such as human attribute translation and style modifications.
% % summarize existing methods:并体现矛盾，即使小的局部修改需要这样整个迭代过程吗
% All these methods follow a similar iterative routine to image generation. Even though editing only involves fine-grained modifications, they still require the whole process from noise to an image.
In general, conditional diffusion models manipulate images by injecting guidance information to each step of the inference process, where the guidance information could be generated from CLIP \cite{nichol2021glide,avrahami2022blended}, classifier \cite{dhariwal2021guided,zhao2022egsde}, low-pass filter \cite{choi2021ilvr,zhao2022egsde}, mask \cite{avrahami2022blended}, etc. 
Although effective, these methods' editing speed is pretty slow, e.g., it takes several minutes to edit a 1024 x 1024 image, regardless of how subtle the editing effect could be. The reason is that to edit an image, these methods need to start from a Gaussian noise and inject the guidance information in every step throughout the generation process, which takes a lot of time. 
Some recent works \cite{avrahami2022blended,meng2021sdedit,choi2021ilvr} propose to impose guidance only in some appropriate steps. 
This could marginally accelerate the editing process. Nevertheless, they still require a few steps to be involved, and thus, the assumption of inference time is still high. 

% This paradigm gives us the flexibility to select key steps.
In this work, we take a different viewpoint to leverage a conditional diffusion model for image manipulation.
Unlike existing methods \cite{nichol2021glide,avrahami2022blended,dhariwal2021guided,zhao2022egsde,choi2021ilvr} that directly manipulate images progressively with diffusion models, we train an efficient image manipulator under the guidance of diffusion models. 
Especially, we reuse the diffusion training loss to optimize the image manipulator network. This image manipulator can edit an image with only a single forward step and easily generalize to images in the same domain. Therefore, our framework avoids the expensive time consumption during inference while benefiting from the remarkable generation quality of the diffusion model.
Significantly, when this diffusion model is multi-modal, we can obtain a network that edits images with natural language prompts.
% In summary, our key idea is that we take a conditional diffusion model as guidance rather than the image manipulator.

\begin{figure}[htbp]
    \centering
    \includegraphics[width=.5\textwidth]{figs/t_observation.png}
    \caption{Various timesteps lead to various results}
    \label{t-observation}
\end{figure}

In addition, we observed that passing various time steps leads to various editing results, as shown in Fig.\ref{t-observation}. The red boxes in this figure points out the best result. For different prompt, different timesteps achieve the optimal result. It indicates that choosing the proper timesteps in our framework is especially significant.  
Fortunately, our framework offers us a clear indicator of the critical timesteps. The diffusion gradient flowing to edited images can greatly facilitate us in analyzing which timesteps are crucial. 
We convert the value of the gradient into confidence and then calculate the entropy of the confidence map. 
The intuition is that the lower the value, the higher the quality of image-wise guidance provided by the diffusion model.
Therefore, we propose a step-pruning strategy based on the entropy of the gradient confidence map. 
This strategy helps us find the most critical time steps, which not only improves our training efficiency but also improves the quality of image manipulation

% summary
In summary, our contributions are three manifolds:
\begin{itemize}
  \item We propose a novel image editing paradigm by passing diffusion gradient to another image manipulator network. This paradigm supports efficient and effective editing with only one forward step.
  \item With the help of our paradigm, we design the timestep selection strategy from the perspective of information entropy. Based on this, we can train our image editing network more efficiently.
  \item Our experiments demonstrate our method's effectiveness and efficiency in both the qualitative and the quantitative aspects.
\end{itemize}




==> legacy/02_related.tex <==
\section{Related Work}
\label{sec:related}
% Multi-modal diffusion models

% Image Editing
Image editing is modifying an input image using an auxiliary input, such as a scribble, mask, reference image, etc.
Recently, text-driven image manipulations have become very popular because textual prompts are intuitive and easily accessible. They usually utilize a joint image-text representation. 
CLIP is a multi-modal space that contains extremely rich semantics as it is trained using its millions of text-image pairs. 
It has demonstrated good power on different tasks, such as latent space manipulation, domain adaptation, and style transfer.

Another type of multi-modal model that has gained a lot of attention is the text-image generative model. 
Several large-scale text-image models have advanced the generation of images conditioned on plain text, such as Imagen, DALL-E2, Parti, and latent diffusion.
The unprecedented ability of semantic generation benefits from stable training and mode cover of the diffusion model.
Diffusion models consist of two processes, the diffusion process gradually perturbs the data distribution to gaussian noise distribution, while the reverse diffusion process recovers data distribution from the noise. 
In the process of reverse diffusion, usually, a model with a large number of parameters will participate in hundreds of iterative computations.

Most image editing methods using the diffusion model tweak the reverse diffusion process. 
For example, \cite{dhariwal2021guided,zhao2022egsde} updates the predicted distribution with the gradient from a classifier to guide the generation process. 
On this basis, a mask can be added to limit the region of the generation\cite{avrahami2022blended}. 
Replacing the low-frequency information of the intermediate result with that of reference image\cite{choi2021ilvr} allows us to condition structural information of the final output.
We could also condition with a stroke image by adding intermediate noises to the stroke image and then denoising it\cite{meng2021sdedit}.
It is also possible to combine it with CLIP and use reverse diffusion to synthesize images from different domains.

Different from previous methods, we aim to solve the limitation of the resources using diffusion models and explore the redundancy of timesteps. 
By distilling high-quality gradients from the diffusion model to a downstream image manipulation framework, we can use diffusion multimodal properties more efficiently and with low overhead 
% Unlike previous works, our method requires textual input only, by using the spatial information from the
% internal layers of the generative model itself. This offers the user a much more intuitive editing experience of
% modifying local or global details by merely modifying the text prompt.



% Numerous works [11, 16, 42, 25, 26, 30, 31, 34, 49, 9, 13, 36] significantly advanced the generation of
% images conditioned on plain text, known as text-to-image synthesis. Several large-scale text-image models
% have recently emerged, such as Imagen [38], DALL-E2 [33], and Parti [48], demonstrating unprecedented
% semantic generation. However, these models do not provide control over a generated image, specifically using
% text guidance only. Changing a single word in the original prompt associated with the image often leads to
% a completely different outcome. For instance, adding the adjective “white” to “dog” often changes the dog’s
% shape. To overcome this, several works [28, 4] assume that the user provides a mask to restrict the area in
% which the changes are applied








==> legacy/02_related_v1.tex <==
\section{Related Work}
\label{sec:related}
% Multi-modal diffusion models

% Image Editing
Image editing \cite{isola2017image,choi2018stargan,chen2019homomorphic,chen2020domain,patashnik2021styleclip,kwon2022clipstyler,kocasari2022stylemc,avrahami2022blended,avrahami2022blendedlatent,choi2021ilvr,meng2021sdedit,zhao2022egsde,hertz2022prompt,kawar2022imagic,ruiz2022dreambooth} is modifying an input image using an auxiliary input, such as a scribble, mask, reference image, etc.
Recently, text-driven image manipulations \cite{patashnik2021styleclip,kwon2022clipstyler,kocasari2022stylemc,avrahami2022blended,avrahami2022blendedlatent, hertz2022prompt,kawar2022imagic,ruiz2022dreambooth,gal2022stylenada} have become very popular because textual prompts are intuitive and easily accessible. 
These methods \cite{kwon2022clipstyler,kim2022diffusionclip,patashnik2021styleclip,kocasari2022stylemc,gal2022stylenada,avrahami2022blended} usually utilize a joint image-text semantic space. 
One of the famous image-text semantic spaces is CLIP \cite{radford2021CLIP}, a multi-modal space that contains extremely rich semantics as it is trained using its millions of text-image pairs. 
It has demonstrated good power on different tasks, such as latent space manipulation\cite{patashnik2021styleclip}, domain adaptation\cite{gal2022stylenada}, and style transfer\cite{kwon2022clipstyler}.

Another type of multi-modal model that has gained a lot of attention is the text-image generative model. 
Several large-scale text-image models have advanced the generation of images conditioned on plain text, such as Imagen\cite{saharia2022imagen}, DALL-E2\cite{ramesh2022dalle2}, Parti, and latent diffusion\cite{rombach2022stablediffusion}.
The unprecedented ability of semantic generation benefits from stable training and mode cover of the diffusion model\cite{ho2020ddpm,sohl2015deep}.
Diffusion models consist of two processes, the diffusion process gradually perturbs the data distribution to gaussian noise distribution, while the reverse diffusion process recovers data distribution from the noise. 
In the process of reverse diffusion, usually, a model with a large number of parameters will participate in hundreds of iterative computations.

Most image editing methods using the diffusion model tweak the reverse diffusion process\cite{zhao2022egsde,meng2021sdedit,avrahami2022blended,avrahami2022blendedlatent,choi2021ilvr,lugmayr2022repaint,dhariwal2021guided, ho2022classifier}. 
For example, \cite{dhariwal2021guided,zhao2022egsde} updates the predicted distribution with the gradient from a classifier to guide the generation process. 
On this basis, a mask can be added to limit the region of the generation\cite{avrahami2022blended}. 
Replacing the low-frequency information of the intermediate result with that of reference image\cite{choi2021ilvr} allows us to condition structural information of the final output.
We could also condition with a stroke image by adding intermediate noises to the stroke image and then denoising it\cite{meng2021sdedit}.
It is also possible to combine it with CLIP and use reverse diffusion to synthesize images from different domains\cite{kim2022diffusionclip}.

Another way to use the power of the diffusion model is to mix it as a prior with other conditional models \cite{graikos2022diffusion, poole2022dreamfusion}. 
This condition model could be a differentiable face classifier and mixing it with a diffusion model can take advantage of the generative power of a diffusion model to generate specific classes of samples for it\cite{graikos2022diffusion}. 
% dreamfusion
On the other hand, \cite{poole2022dreamfusion} utilizes differentiable image parameterization \cite{mordvintsev2018differentiable}  and defines this conditional model as a 3D rendering process \cite{mildenhall2020nerf} to generate 3D assets from text.
Different from utilizing fixed conditional models \cite{graikos2022diffusion,poole2022dreamfusion}, we define this conditional model as an image-to-image translation model, and explore a new scenario where this conditional model is optimized under the guidance of diffusion models. 
This model after optimization can be independent of the diffusion model, thus enabling more efficient image editing.











==> legacy/03_background.tex <==
\section{Background}
\label{background}
% Multi-modal diffusion models

%%%% background: diffusion model as plug-and-play prior
\subsection{Diffusion models}

Diffusion models are latent-variable generative models that define a Markov chain of diffusion steps to add random noise to data slowly and then learn to reverse the diffusion process to construct desired data samples from the noise.\cite{sohl2015deep,ho2020ddpm}.  

Given data sampled from a real data distribution $x_0 \sim q(x)$, the forward diffusion process is defined to add a small amount of Gaussian noise with variance $\beta_t \in (0,1)$ to the sample in $T$ steps, producing a series of noisy latents $x_1,...,x_T$.
\begin{equation}
\small
\begin{aligned}
q(x_t\mid x_{t-1}) = \mathcal{N}(x_t;\sqrt{1-\beta_t}x_{t-1},\beta_tI) \\ q(x_{1:T}\mid x_0) = \prod_{t=1}^T{q(x_t\mid x_{t-1})}
\end{aligned}
\label{E1}
\end{equation}

The process slowly removes structure from data $x_0$, and eventually when $T \rightarrow \infty$, $x_T$ is equal to an isotropic Gaussian distribution.

A notable property of the diffusion process is $x_t$ at any time step can be sampled in a closed form:
\begin{equation}
\small
\begin{aligned}
q(x_t\mid x_0) = \mathcal{N}(x_t;\sqrt{\bar{\alpha}_t}x_0,(1-\bar{\alpha}_t)I) \\
x_t=\sqrt{\bar{\alpha}_t}x_0+\sqrt{1-\bar{\alpha}_t}\epsilon
\end{aligned}
\label{E2}
\end{equation}
where $\alpha_t = 1 - \beta_t$ and $\bar{\alpha}_t = \prod_{i=1}^t\alpha_i$

The computation of reverse diffusion process $q(x_{t-1}\mid x_t)$ requires us to use the entire dataset. 
Therefore, diffusion models learn a model $p_{\theta}$ to approximate the posterior distribution:
\begin{equation}
\small
\begin{aligned}
p_{\theta}(x_{t-1}\mid x_{t}) = \mathcal{N}(x_t;\mu_\theta(x_t, t),\Sigma_\theta(x_t, t)) \\ p_{\theta}(x_{0:T}) = p(x_T)\prod_{t=1}^T{p_{\theta}(x_{t-1}\mid x_{t})}
\end{aligned}
\label{E3}
\end{equation}

Especially, $p_\theta$ is to approximate the $q(x_{t-1}|x_{t}, x_0):= \mathcal{N}(\widetilde{\mu}_t, \widetilde{\beta}_tI)$, which is a posterior distribution derived from the forward process, and:
\begin{equation}
\small
\begin{aligned}
\widetilde{\mu}_t:=\frac{1}{\sqrt{\alpha_t}}(x_t-\frac{\beta_t}{\sqrt{1-{\bar{\alpha}_t}}}\epsilon_t) \\
\widetilde{\beta}_t:=\frac{1-\bar{\alpha}_{t-1}}{1-\bar{\alpha}_t}\beta_t
\end{aligned}
\label{E4}
\end{equation}

Because $x_t$ is available as input at training time, we can reparameterize the Gaussian noise term instead to make it predict $\epsilon_t$ from the input $x_t$.
Finally, we can train this latent-variable model with simplified evidence lower bound (ELBO) that ignores the weighting term for each time step $t$ \cite{ho2020ddpm}:
\begin{equation}
\small
\begin{aligned}
\mathcal{L}_t=\mathbb{E}_{t,\epsilon}[\left \Vert \epsilon - \epsilon_{\theta}(\sqrt{\bar{\alpha}_t}\mathbf{x} + \sqrt{1-\bar{\alpha}_t}\epsilon,t) \right \Vert^2_2]
\end{aligned}
\label{E5}
\end{equation}

\subsection{Diffusion models as prior}
%%%%%%%% Diffusion Prior
% diffusion model 也可以off-the-shelf的使用，作为其他条件模型的先验
Diffusion models can be used as off-the-shelf modules in some scenarios, where one model may serve as a prior for another conditional model.

% 一种经典的场景是：diffusion model作为prior，条件模型为分类器，我们可以利用diffusion model的先验，来实现条件生成
A typical example is that we have a diffusion model $p(x)$ trained on MNISIT images, and an off-the-shelf classifier $c(x, y)$ where $y$ is the class label.
Then we can use the diffusion model to generate data of class $y$ for the classifier $c(x, y)$.

In theory, this means that we want to deduce $p(x\mid y)$ given $p(x)$ and $c(x,y)$.
To approximate the posterior distribution $p(x|y)$, we can introduce an approximate variational posterior $q(x)$ by minimizing
\begin{equation}
\small
\begin{aligned}
F = -\mathbb{E}_{q(\mathbf{x})}[\log{p(\mathbf{x})}-\log{q(\mathbf{x})}]-\mathbb{E}_{q(\mathbf{x})}[\log{c(\mathbf{x},\mathbf{y})}]
\end{aligned}
\label{E6}
\end{equation}
%使用prior的结果
Extending this formula to the scenario of diffusion model with latent variable $x_1,...,x_T$, we define this approximate variational posterior $q(x)$ as point estimate $q(\mathbf{x})=\delta(\mathbf{x}-\eta) $\cite{graikos2022diffusion}, and then:
\begin{equation}
\small
\begin{aligned}
F = \sum_t\mathbb{E}_{\epsilon\sim \mathcal{N}(0,I)}[\left \Vert \epsilon - \epsilon_{\theta}(\mathbf{x_t},t) \right \Vert^2_2] -\mathbb{E}_{q(\mathbf{x})}[\log{c(\mathbf{\eta},\mathbf{y})}] \\ \mathbf{x}_t= \sqrt{\bar{\alpha}_t}\eta + \sqrt{1-\bar{\alpha}_t}\epsilon
\end{aligned}
\label{E7}
\end{equation}
This equation optimizes $\eta$ which has the same dimensionality as data. 
We can regard this equation as sampling pixels using diffusion models to satisfy the condition $y$.

Especially, when $c(\mathbf{x},\mathbf{y})$ is a hard and non-differentiable conditional model, say a deterministic function $x=f(y)$. 
For example, $f()$ can be a latent-variable model that takes latent $y$ as input and generates a sample $x$.
Another example is that we can also use techniques of differentiable image parameterization. 
In \cite{poole2022dreamfusion}, $y$ can be parameters of a 3D volume, and $f$ is a volumetric renderer. 
Then the gradient descent steps will be performed with respect to $\mathbf{y}$ on
\begin{equation}
\small
\begin{aligned}
\sum_t\mathbb{E}_{\epsilon\sim \mathcal{N}(0,I)}[\left \Vert \epsilon - \epsilon_{\theta}(\sqrt{\bar{\alpha}_t}f(\mathbf{y}) + \sqrt{1-\bar{\alpha}_t}\epsilon,t) \right \Vert^2_2]
\end{aligned}
\label{E8}
\end{equation}
We can regard this equation as sampling $y$ instead of directly sampling images using diffusion models.

% 加一句实际上不会每一代都计算所有t
In practice, optimizing simultaneously for all $t$ makes it difficult to guide the sample towards a mode, and thus existing methods eighter anneal $t$ from high to low values \cite{graikos2022diffusion} or random select $t$ \cite{poole2022dreamfusion}.
So the actual optimization process is slightly changed to
\begin{equation}
\small
\begin{aligned}
\mathbb{E}_{\epsilon,t}[\left \Vert \epsilon - \epsilon_{\theta}(\sqrt{\bar{\alpha}_t}f(\mathbf{y}) + \sqrt{1-\bar{\alpha}_t}\epsilon,t) \right \Vert^2_2]
\end{aligned}
\label{E8}
\end{equation}

==> legacy/03_background_v1.tex <==
\section{Preliminary}
\label{sec:preliminary}
% Multi-modal diffusion models

%%%% background: diffusion model as plug-and-play prior
\subsection{Diffusion Models}

Diffusion models are latent-variable generative models that define a Markov chain of diffusion steps to add random noise to data slowly and then learn to reverse the diffusion process to construct desired data samples from the noise \cite{sohl2015deep,ho2020ddpm}.  

Suppose the data distribution is $q(x_0)$ where the index $0$ denotes the original data. Given a training data sample $x_0\sim q(x_0)$, the forward diffusion process aims to produce a series of noisy latents $x_1,x_2,\cdots,x_T$ by the following Markovian process,
\begin{equation}
q(x_t\mid x_{t-1}) = \mathcal{N}(x_t;\sqrt{1-\beta_t}x_{t-1},\beta_t\mathbf{I}), \forall t\in [T],
\label{eq:forward}
\end{equation}
where $T$ is the step number of the diffusion process, $[T]=\{1,2,\cdots, T\}$ denotes the set of the index, $\beta_t\in(0,1)$ represents the variance in the diffusion process, $\mathbf{I}$ is the identity matrix with the same dimensions as the input data $x_0$, and $\mathcal{N}(x;\mu,\sigma)$ means the normal distribution with mean $\mu$ and covariance $\sigma$.

% Given data sampled from a real data distribution $x_0 \sim q(x)$, the forward diffusion process is defined to add a small amount of Gaussian noise with variance $\beta_t \in (0,1)$ to the sample in $T$ steps, producing a series of noisy latents $x_1,...,x_T$.
% \begin{equation}
% \small
% \begin{aligned}
% q(x_t\mid x_{t-1}) = \mathcal{N}(x_t;\sqrt{1-\beta_t}x_{t-1},\beta_tI) \\ q(x_{1:T}\mid x_0) = \prod_{t=1}^T{q(x_t\mid x_{t-1})}
% \end{aligned}
% \label{E1}
% \end{equation}

% The process slowly removes structure from data $x_0$, and eventually when $T \rightarrow \infty$, $x_T$ is equal to an isotropic Gaussian distribution.

% Since $q(x_{1:T}\mid x_0) = \prod_{t=1}^T{q(x_t\mid x_{t-1})}$, we have 
% \begin{equation}
%     q(x_t\mid x_0) = \mathcal{N}(x_t;\sqrt{\bar{\alpha}_t}x_0,(1-\bar{\alpha}_t)\mathbf{I}),
% \end{equation}
% where $\bar{\alpha}_t = \prod_{i=1}^t\alpha_i$ and $\alpha_t = 1 - \beta_t$. Thus, $x_t$ at any timestep can be computed in a closed form by using the reparameterization trick as follows,
% \begin{equation}
% x_t=\sqrt{\bar{\alpha}_t}x_0+\sqrt{1-\bar{\alpha}_t}\epsilon_t,
% \label{E2}
% \end{equation}
% where $\epsilon_t$ is sampled from the standard normal distribution and has the same dimensions as $x_0$. Hence, the forward process slowly removes structure from data $x_0$, and eventually when $T \rightarrow \infty$, the distribution of $x_T$ is equal to the standard normal distribution.

To generate a new data sample, diffusion models sample $x_T$ from the standard normal distribution and then gradually remove noise by the intractable reverse distribution $q(x_{t-1}\mid x_t)$. Diffusion models learn a neural network $p_{\theta}$ parameterized by $\theta$ to approximate the reverse distribution as follows,
\begin{equation}
% \small
% \begin{aligned}
p_{\theta}(x_{t-1}\mid x_{t}) = \mathcal{N}(x_{t-1};\mu_\theta(x_t, t),\Sigma_\theta(x_t, t)), 
% \\ p_{\theta}(x_{0:T}) = p(x_T)\prod_{t=1}^T{p_{\theta}(x_{t-1}\mid x_{t})}.
% \end{aligned}
\label{E3}
\end{equation}
where $\mu_\theta$ and $\Sigma_\theta$ are the trainable mean and covariance functions, respectively.

% Especially, $p_\theta$ approximates the $q(x_{t-1}|x_{t}, x_0):= \mathcal{N}(\widetilde{\mu}_t, \widetilde{\beta}_tI)$, which is a posterior distribution derived from the forward process, and:
In \cite{ho2020ddpm}, $\Sigma_\theta$ is simply set as a fixed constant, and $\mu_\theta$ is reformulated as a function of noise as follows,
\begin{equation}
% \small
% \begin{aligned}
\mu_\theta(x_t,t)=\frac{1}{\sqrt{\alpha_t}}\left(x_t-\frac{\beta_t}{\sqrt{1-{\bar{\alpha}_t}}}\epsilon_\theta(x_t, t)\right), \\
% \widetilde{\beta}_t:=\frac{1-\bar{\alpha}_{t-1}}{1-\bar{\alpha}_t}\beta_t.
% \end{aligned}
% \label{E4}
\end{equation}
where $\epsilon_\theta$ is used to predict noise $\epsilon_t$ from $x_t$.

% Because $x_t$ is available as input at training time, we can reparameterize the Gaussian noise term instead to make it predict $\epsilon_t$ from the input $x_t$.
Finally, the diffusion model is trained with simplified evidence lower bound (ELBO) that ignores the weighting term for each timestep $t$ as follows,
\begin{equation}
\mathcal{L}_t(\theta)=\mathbb{E}_{x_0, t,\epsilon}\left[ \left\Vert \epsilon_t - \epsilon_{\theta}(x_t, t) \right\Vert^2_2\right].
\label{E5}
\end{equation}

\subsection{Diffusion Models as Prior}
\label{Diffusion-models-as-prior}
%%%%%%%% Diffusion Prior
% diffusion model 也可以off-the-shelf的使用，作为其他条件模型的先验
According to \cite{graikos2022diffusion}, diffusion models can also be used as off-the-shelf modules in some scenarios, where it $p(x)$ may serve as a prior for another conditional model $c(x, y)$, \ie we can deduce $p(x\mid y)$ given $p(x)$ and $c(x,y)$.
When $c(\mathbf{x},\mathbf{y})$ is a hard and non-differentiable conditional model, say a deterministic function $x=f(y)$. We optimize $\mathbf{y}$ to minimize
\begin{equation}
\small
\begin{aligned}
\sum_t\mathbb{E}_{\epsilon\sim \mathcal{N}(0,I)}[\left \Vert \epsilon - \epsilon_{\theta}(\sqrt{\bar{\alpha}_t}f(\mathbf{y}) + \sqrt{1-\bar{\alpha}_t}\epsilon,t) \right \Vert^2_2].
\end{aligned}
\label{E8}
\end{equation}
For example, $f()$ is a latent-variable model that takes latent $y$ as input and generates a sample $x$. 
We can regard this equation as sampling $\mathbf{y}$ instead of directly sampling images using diffusion models, and inputting $\mathbf{y}$ to this conditional model, we will get a sample from the diffusion model.
One well-known example is DreamFusion \cite{poole2022dreamfusion} where $y$ is the parameters of a 3D volume, and $f$ is a volumetric renderer. It can achieve text-to-3D assets generation.

% 加一句实际上不会每一代都计算所有t
In practice, optimizing simultaneously for all $t$ makes it difficult to guide the sample towards a mode. Thus existing methods eighter anneal $t$ from high to low values \cite{graikos2022diffusion}, or random select $t$ \cite{poole2022dreamfusion}.
So the actual optimization process is slightly changed to
\begin{equation}
\small
\begin{aligned}
\mathbb{E}_{\epsilon,t}[\left \Vert \epsilon - \epsilon_{\theta}(\sqrt{\bar{\alpha}_t}f(\mathbf{y}) + \sqrt{1-\bar{\alpha}_t}\epsilon,t) \right \Vert^2_2]
\end{aligned}
\label{E9}
\end{equation}

==> legacy/03_method.tex <==
\section{Method}
\label{sec:method}
%%%% background: diffusion model as plug-and-play prior
\subsection{Diffusion Models}

Diffusion models are latent-variable generative models that define a Markov chain of diffusion steps to slowly add random noise to data and then learn to reverse the diffusion process to construct desired data samples from the noise.\cite{sohl2015deep,ho2020ddpm}.  

Given data sampled from a real data distribution $x_0 \sim q(x)$, the forward diffusion process is defined to add a small amount of Gaussian noise with variance $\beta_t \in (0,1)$ to the sample in $T$ steps, producing a series of noisy latents $x_1,...,x_T$.
\begin{equation}
\small
\begin{aligned}
q(x_t\mid x_{t-1}) = \mathcal{N}(x_t;\sqrt{1-\beta_t}x_{t-1},\beta_tI) \\ q(x_{1:T}\mid x_0) = \prod_{t=1}^T{q(x_t\mid x_{t-1})}
\end{aligned}
\label{E2}
\end{equation}

The process slowly removes structure from data $x_0$ and eventually when $T \rightarrow \infty$, $x_T$ is equal to an isotropic Gaussian distribution.

A notable property of the diffusion process is $x_t$ at any time step can be sampled in a closed form:
\begin{equation}
\small
\begin{aligned}
q(x_t\mid x_0) = \mathcal{N}(x_t;\sqrt{\bar{\alpha}_t}x_0,(1-\bar{\alpha}_t)I) \\
x_t=\sqrt{\bar{\alpha}_t}x_0+\sqrt{1-\bar{\alpha}_t}\epsilon
\end{aligned}
\label{E2}
\end{equation}
where $\alpha_t = 1 - \beta_t$ and $\bar{\alpha}_t = \prod_{i=1}^t\alpha_i$

The reverse diffusion process $q(x_{t-1}\mid x_t)$ requires us to use the entire dataset and therefore diffusion models learn a model $p_{\theta}$ to approximate the posterior distribution:
\begin{equation}
\small
\begin{aligned}
p_{\theta}(x_{t-1}\mid x_{t}) = \mathcal{N}(x_t;\mu_\theta(x_t, t),\Sigma_\theta(x_t, t)) \\ p_{\theta}(x_{0:T}) = p(x_T)\prod_{t=1}^T{p_{\theta}(x_{t-1}\mid x_{t})}
\end{aligned}
\label{E2}
\end{equation}

Especially, $p_\theta$ is to approximate the $q(x_{t-1}|x_{t}, x_0):= \mathcal{N}(\widetilde{\mu}_t, \widetilde{\beta}_tI)$, which is a posterior distribution derived from the forward process, and:
\begin{equation}
\small
\begin{aligned}
\widetilde{\mu}_t:=\frac{1}{\sqrt{\alpha_t}}(x_t-\frac{\beta_t}{\sqrt{1-{\bar{\alpha}_t}}}\epsilon_t) \\
\widetilde{\beta}_t:=\frac{1-\bar{\alpha}_{t-1}}{1-\bar{\alpha}_t}\beta_t
\end{aligned}
\label{E2}
\end{equation}

Because $x_t$ is available as input at training time, we can reparameterize the Gaussian noise term instead to make it predict $\epsilon_t$ from the input $x_t$ at the time step.
Finally, Ho et al \cite{ho2020ddpm} train this latent-variable model with simplified evidence lower bound (ELBO) that ignores the weighting term for each time step $t$:
\begin{equation}
\small
\begin{aligned}
\mathcal{L}_t=\mathbb{E}_{t\sim [1,T],\epsilon \sim \mathcal{N}(0,I)}[\left \Vert \epsilon - \epsilon_{\theta}(\sqrt{\bar{\alpha}_t}\mathbf{x} + \sqrt{1-\bar{\alpha}_t}\epsilon,t) \right \Vert^2_2]
\end{aligned}
\label{E1}
\end{equation}


 
% Diffusion model training can thereby be viewed as either learning a latent-variable model \cite{sohl2015deep,ho2020ddpm}, or learning a sequence of score functions corresponding to noisier versions of the data \cite{song2019score1, song2020score2}. 
% We will use $p_{\phi}(z_t; t)$ to denote the approximate marginal distribution whose score function is given by $s_{\phi}(z_t; t) = -\phi(z_t; t)/\sigma_t$.



% The predicted noise can be related to a predicted score function for the smoothed density $\nabla x_t \log{p(x_t)}$ through Tweedie’s formula \cite{robbins1992empirical}: $\theta(x_t; t) = -\sqrt{1-\bar{\alpha}_t} s_{\theta}(x_t; t)$.


\subsection{Diffusion Models as Prior}
% %定义：使用prior
Generative models can be used as priors. 
Assume we have a prior $p(x)$ over high-dimensional data $x$ and we wish to perform inference in a model that involves this prior and a constraint $c(x, y)$ on $x$ given some additional information $y$. 
In other words, we wish to use unconditional models to realize conditional generation.
For example, a generative model trained on CIFAR-10 images might define p(x), while the constraint c(x, y) may be the probability of class y under an off-the-shelf classifier.
This means we want to deduce $p(x\mid y)$ given $p(x)$ and $c(x,y)$. 
To approximate the posterior distribution $p(x|y)$, we can introduce an approximate variational posterior $q(x)$ by minimizing
\begin{equation}
\small
\begin{aligned}
F = -\mathbb{E}_{q(\mathbf{x})}[\log{p(\mathbf{x})}-\log{q(\mathbf{x})}]-\mathbb{E}_{q(\mathbf{x})}[\log{c(\mathbf{x},\mathbf{y})}]
\end{aligned}
\label{E2}
\end{equation}
%使用prior的结果
When this prior is a diffusion model with latent variable $x_1,...,x_T$, the approximate variational posterior $q(x)$ is defined as point estimate $q(\mathbf{x})=\delta(\mathbf{x}-\eta)$ \cite{graikos2022diffusion}. This optimization turns into:
\begin{equation}
\small
\begin{aligned}
F = \sum_t\mathbb{E}_{\epsilon\sim \mathcal{N}(0,I)}[\left \Vert \epsilon - \epsilon_{\theta}(\mathbf{x_t},t) \right \Vert^2_2] -\mathbb{E}_{q(\mathbf{x})}[\log{c(\mathbf{\eta},\mathbf{y})}] \\ \mathbf{x}_t= \sqrt{\bar{\alpha}_t}\eta + \sqrt{1-\bar{\alpha}_t}\epsilon
\end{aligned}
\label{E5}
\end{equation}
Here we aim to optimize $\eta$ that has the same dimensionality as data, and we can regard this equation as sampling pixels using diffusion models to satisfy the constraint given condition $y$.

Especially, when constraints $c(\mathbf{x},\mathbf{y})$ is a hard and non-differentiable constraint, say a deterministic function $x=f(y)$. 
Then the gradient descent steps will be performed with respect to $\mathbf{y}$ on
\begin{equation}
\small
\begin{aligned}
\sum_t\mathbb{E}_{\epsilon\sim \mathcal{N}(0,I)}[\left \Vert \epsilon - \epsilon_{\theta}(\sqrt{\bar{\alpha}_t}f(\mathbf{y}) + \sqrt{1-\bar{\alpha}_t}\epsilon,t) \right \Vert^2_2]
\end{aligned}
\label{E8}
\end{equation}
Since image $x$ is determined by $y$, we can regard this equation as sampling $y$ instead of directly sampling pixels using diffusion models.
When we involve techniques of differentiable image parameterization, $y$ becomes the parameters of a network, $f$ becomes a differentiable generator, and it transforms parameters $\mathbf{y}$ to create an image $\mathbf{x} = f(y)$. 
For example, \cite{poole2022dreamfusion} define $y$ as parameters of a NERF and generate a 3D object using a 2D diffusion prior.

Although there have been good results using this method, there are two essential points that have not been sufficiently discussed. 
First is the constraint. We aim to explore a new situation of using diffusion prior, where we use equation \eqref{E8} to optimize a differentiable generator $f$. 
For example, $y$ is the input image and $f$ is an image-to-image translation network, and the output image $x$ is sampled indirectly by optimizing the $f$.
We can regard this as optimizing a translation, after which images will change toward the mode defined by the text description of the multi-modal diffusion model.

Second is the time step, each optimization step requires us to compute for all $t$ simultaneously but it is difficult to guide the sample towards a mode in image generation applications\cite{graikos2022diffusion}. 
Therefore, existing works either anneal $t$ from high values to low values \cite{graikos2022diffusion} or randomly pick $t$ \cite{poole2022dreamfusion}.
However, when some of the time steps are useless and even harmful to the optimization process, these strategies become sub-optimal.
This phenomenon is very common in image editing and different editing even may be sensitive to different time steps, so we need a carefully designed strategy to help us rule out redundant time steps.

\subsection{Implementation details}
% %分析：这本质上做的事情，是将sample pixel变成了sample其他东西
% Using diffusion models, we can regard this equation as sampling latent instead of pixels.
% %举例说明：
% For example, if the constraint is a latent variable model, 
% %举例：用dreamfusion作为一个例子，将sample pixel变成了sample 3D volume的参数
% Especially when we involve techniques of differentiable image parameterization, this equation process could be used to optimize the parameters of a network. 
% At this time this function $f$ becomes a differentiable generator, and it transforms parameters $\mathbf{y}$ to create an image $\mathbf{x} = f(y)$. 
% If this network is a 3D model\cite{poole2022dreamfusion}, then we can even generate 3D object using this 2D diffusion prior.

% In this work, we will explore more flexible usage of diffusion prior. 
% For example, we are using the gradient of the diffusion model to optimize $f(\cdot)$. 
% The intuition is that our goal is to optimize a kind of translation,  after which y will conform to the distribution of diffusion prior.

% %定义：使用prior的一般优化目标
% To approximate the posterior distribution $p(x|y)$, they introduce an approximate variational posterior $q(x)$ by minimizing:
% \begin{equation}
% \small
% \begin{aligned}
% F = -\mathbb{E}_{q(\mathbf{x})}[\log{p(\mathbf{x})}-\log{q(\mathbf{x})}]-\mathbb{E}_{q(\mathbf{x})}[\log{c(\mathbf{x},\mathbf{y})}]
% \end{aligned}
% \label{E2}
% \end{equation}
% %问题：diffusion prior的p(x)不可得
% Here, calculating $p(\mathbf{x})$ would require an intractable integration over latent variables $\mathbf{h}=(\mathbf{x}_T,...,\mathbf{x}_1)$:
% \begin{equation}
% \small
% \begin{aligned}
% p(\mathbf{x})=\int_\mathbf{h}p(\mathbf{x}_T,\mathbf{x}_{T-1},...,\mathbf{x}_1,\mathbf{x}_0=\mathbf{x})d\mathbf{x}_T...d\mathbf{x}_1
% \end{aligned}
% \label{E3}
% \end{equation}
% %推导：使用latent variable的形式代换
% To solve this, we can first rewrite this free energy using joint distribution:
% \begin{equation}
% \small
% \begin{aligned}
% F = -\mathbb{E}_{q(\mathbf{x})q(\mathbf{h|x})}[\log{p(\mathbf{x,h})}-\log{q(\mathbf{x})q(\mathbf{h|x})}] \\ -\mathbb{E}_{q(\mathbf{x})}[\log{c(\mathbf{x},\mathbf{y})}]
% \end{aligned}
% \label{E4}
% \end{equation}
% %推导：使用点估计，以及DDPM中的推导和简化，得打优化目标
% Secondly, according to the definition of the posterior distribution in diffusion models, we can compute this distribution. 
% Next, we could define the approximate variational posterior as point estimate $q(\mathbf{x})=\delta(\mathbf{x}-\eta)$, and using the same idea and reparameterization as \cite{ho2020ddpm}, we could rewrite \eqref{E4} as:
% \begin{equation}
% \small
% \begin{aligned}
% F = \sum_t\mathbb{E}_{\epsilon\sim \mathcal{N}(0,I)}[\left \Vert \epsilon - \epsilon_{\theta}(\mathbf{x_t},t) \right \Vert^2_2] \\ -\mathbb{E}_{q(\mathbf{x})}[\log{c(\mathbf{\eta},\mathbf{y})}], \mathbf{x}_t= \sqrt{\bar{\alpha}_t}\eta + \sqrt{1-\bar{\alpha}_t}\epsilon
% \end{aligned}
% \label{E5}
% \end{equation}
% %泛化：在c(x, y)为determinitic function时的优化目标
% Especially, when constraints $c(\mathbf{x},\mathbf{y})$ is a hard and non-differentiable constraint, say a deterministic function. 
% Then the gradient descent steps will be performed with respect to $\mathbf{y}$ on
% \begin{equation}
% \small
% \begin{aligned}
% \left \Vert \epsilon - \epsilon_{\theta}(\sqrt{\bar{\alpha}_t}f(\mathbf{y}) + \sqrt{1-\bar{\alpha}_t}\epsilon,t) \right \Vert^2_2
% \end{aligned}
% \label{E6}
% \end{equation}
% %分析：这本质上做的事情，是将sample pixel变成了sample其他东西
% Using diffusion models, we can regard this equation as sampling latent instead of pixels.
% %举例说明：
% For example, if the constraint is a latent variable model, this equation aims to optimize a latent through which it will generate a sample conforming to the prior diffusion distribution. 
% %举例：用dreamfusion作为一个例子，将sample pixel变成了sample 3D volume的参数
% Especially when we involve techniques of differentiable image parameterization, this equation process could be used to optimize the parameters of a network. 
% At this time this function $f$ becomes a differentiable generator, and it transforms parameters $\mathbf{y}$ to create an image $\mathbf{x} = f(y)$. 
% If this network is a 3D model\cite{poole2022dreamfusion}, then we can even generate 3D object using this 2D diffusion prior.

% In this work, we will explore more flexible usage of diffusion prior. 
% For example, we are using the gradient of the diffusion model to optimize $f(\cdot)$. 
% The intuition is that our goal is to optimize a kind of translation,  after which y will conform to the distribution of diffusion prior.

% \subsection{Image Editing using Diffusion Prior}
% In this section, we will first elaborate on the cost problem of traditional diffusion-based image editing methods and propose a new image editing method that uses the diffusion model as prior. 
% This method can save costs compared to traditional methods. 
% However, 
% % % 分析：在以上例子中，我们使用text diffusion，因此可以直接传入condition，再加上latent的形式c(x,y), 我们实际上在使用diffusion决定我们需要去approxiamte的分布，用c(x,y)来决定我们优化过程实际所发生的位置。因此，以上工作只讨论了优化发生在latent variable上的情况
% % The method uses a text-conditioned diffusion model, and a deterministic function. We actually pre-define a text description condition, and so the diffusion prior actually determines the distribution we want to approximate(e.g, what sample we want to obtain), while constraint function determine the place this approximation process happens(e.g, by optimizing what target). These methods only discuss replace sample pixels with sample latent variables. 

% % % 引入: 如果我们不只限于在latent variable，改变sample发生的位置，我们就可以将diffusion prior的知识传播到其他地方，例如将sample/optimize过程移至网络中，让网络负责学习编辑过程。并且，网络在优化后也不借助diffusion process来完成一些引用
% % Intuitively, we could change the place that sampling/optimization happens to change the place the knowledge of diffusion models that propagate to. 
% % For example, if we could optimize image editing model using this gradient, then the model can perform image editing itself without access to diffusion model.

% % 这就是知识蒸馏的思想，一些分析，为什么图像编辑摆脱denoising process是合理的，因为实质上diffusion是生成模型，它需要整个过程来保证最后的生成内容，而图像编辑实质上是一种translation，本质上是对原有图像上的semantic information，style information进行修改，而已有的content information我们保留就好，所以使用diffusion process进行编辑，我们需要在生成过程中去人为逆转掉对原有图像content information的改变，而本质上最优的方式是仅仅学习在对应semantic information和style information上的改变就好，因此并不需要整个denoise process.
% Why it is supposed to do so. 
% Diffusion prior as a generative model uses a lot of computation for creation from nothing. However, image editing actually is to translate some information (e.g, style information, attribute information) from the original image and preserves the rest of them (e.g, content information). 
% Using the denoising process of diffusion to do image editing, we inevitably need some operations at each step to reverse some unwanted modifications brought by its generative property, e.g., using a mask to block some changes.
% The optimal method should be only learning the translation that we want it to happen, which is incremental. 
% In this way, we avoid unnecessary changes brought by the generative properties of diffusion models, thus saving a lot of time and calculation.


% % 接下来，为了只学习到translation增量的知识，我们将围绕latent space image manipulation进行讨论，因为在这里一个编辑方向可以被一个latent space的vector所代表。
% In order to become more efficient and learn only one increment, we will discuss latent space image manipulation with diffusion prior, since here editing can be represented by one increment in latent space. 
% We will first use the basic method to use diffusion-prior to optimize another latent of latent variable models
% % 首先，我们选择stylegan的latent space，进行step by step的讨论

\subsection{Our method}
In this section, we will propose a new paradigm of utilizing diffusion prior and apply it to image editing. 
% To demonstrate the generalizability of this paradigm, we discuss two common forms of image editing, image-to-image translation, and latent space image manipulation.
\begin{equation}
\small
\begin{aligned}
\min_{\theta}\sum_t\mathbb{E}_{\epsilon\sim \mathcal{N}(0,I)}[\left \Vert \epsilon - \epsilon_{\theta}(\sqrt{\bar{\alpha}_t}f_\theta(\mathbf{y}) + \sqrt{1-\bar{\alpha}_t}\epsilon,t) \right \Vert^2_2]
\end{aligned}
\label{E8}
\end{equation}

==> legacy/03_method_v2.tex <==
\section{Method}
\label{sec:method}
%%%% background: diffusion model as plug-and-play prior
\subsection{Diffusion Models}

Diffusion models are latent-variable generative models that define a Markov chain of diffusion steps to add random noise to data slowly and then learn to reverse the diffusion process to construct desired data samples from the noise.\cite{sohl2015deep,ho2020ddpm}.  

Given data sampled from a real data distribution $x_0 \sim q(x)$, the forward diffusion process is defined to add a small amount of Gaussian noise with variance $\beta_t \in (0,1)$ to the sample in $T$ steps, producing a series of noisy latents $x_1,...,x_T$.
\begin{equation}
\small
\begin{aligned}
q(x_t\mid x_{t-1}) = \mathcal{N}(x_t;\sqrt{1-\beta_t}x_{t-1},\beta_tI) \\ q(x_{1:T}\mid x_0) = \prod_{t=1}^T{q(x_t\mid x_{t-1})}
\end{aligned}
\label{E1}
\end{equation}

The process slowly removes structure from data $x_0$, and eventually when $T \rightarrow \infty$, $x_T$ is equal to an isotropic Gaussian distribution.

A notable property of the diffusion process is $x_t$ at any time step can be sampled in a closed form:
\begin{equation}
\small
\begin{aligned}
q(x_t\mid x_0) = \mathcal{N}(x_t;\sqrt{\bar{\alpha}_t}x_0,(1-\bar{\alpha}_t)I) \\
x_t=\sqrt{\bar{\alpha}_t}x_0+\sqrt{1-\bar{\alpha}_t}\epsilon
\end{aligned}
\label{E2}
\end{equation}
where $\alpha_t = 1 - \beta_t$ and $\bar{\alpha}_t = \prod_{i=1}^t\alpha_i$

The reverse diffusion process $q(x_{t-1}\mid x_t)$ requires us to use the entire dataset and therefore diffusion models learn a model $p_{\theta}$ to approximate the posterior distribution:
\begin{equation}
\small
\begin{aligned}
p_{\theta}(x_{t-1}\mid x_{t}) = \mathcal{N}(x_t;\mu_\theta(x_t, t),\Sigma_\theta(x_t, t)) \\ p_{\theta}(x_{0:T}) = p(x_T)\prod_{t=1}^T{p_{\theta}(x_{t-1}\mid x_{t})}
\end{aligned}
\label{E3}
\end{equation}

Especially, $p_\theta$ is to approximate the $q(x_{t-1}|x_{t}, x_0):= \mathcal{N}(\widetilde{\mu}_t, \widetilde{\beta}_tI)$, which is a posterior distribution derived from the forward process, and:
\begin{equation}
\small
\begin{aligned}
\widetilde{\mu}_t:=\frac{1}{\sqrt{\alpha_t}}(x_t-\frac{\beta_t}{\sqrt{1-{\bar{\alpha}_t}}}\epsilon_t) \\
\widetilde{\beta}_t:=\frac{1-\bar{\alpha}_{t-1}}{1-\bar{\alpha}_t}\beta_t
\end{aligned}
\label{E4}
\end{equation}

Because $x_t$ is available as input at training time, we can reparameterize the Gaussian noise term instead to make it predict $\epsilon_t$ from the input $x_t$ at the time step.
Finally, Ho et al \cite{ho2020ddpm} train this latent-variable model with simplified evidence lower bound (ELBO) that ignores the weighting term for each time step $t$:
\begin{equation}
\small
\begin{aligned}
\mathcal{L}_t=\mathbb{E}_{t,\epsilon}[\left \Vert \epsilon - \epsilon_{\theta}(\sqrt{\bar{\alpha}_t}\mathbf{x} + \sqrt{1-\bar{\alpha}_t}\epsilon,t) \right \Vert^2_2]
\end{aligned}
\label{E5}
\end{equation}

\subsection{Diffusion Models as Prior}
% %定义：使用prior
Assume we have a prior $p(x)$ over high-dimensional data $x$ and we wish to perform inference in a model that involves this prior and a constraint $c(x, y)$ on $x$ given some additional information $y$. 
% In other words, we wish to use unconditional models to realize conditional generation.
For example, a generative model trained on CIFAR-10 images might define $p(x)$, while the constraint c(x, y) may be the probability of class $y$ under an off-the-shelf classifier.
This means we want to deduce $p(x\mid y)$ given $p(x)$ and $c(x,y)$. In other words, we wish to use unconditional models to realize conditional generation.
To approximate the posterior distribution $p(x|y)$, we can introduce an approximate variational posterior $q(x)$ by minimizing
\begin{equation}
\small
\begin{aligned}
F = -\mathbb{E}_{q(\mathbf{x})}[\log{p(\mathbf{x})}-\log{q(\mathbf{x})}]-\mathbb{E}_{q(\mathbf{x})}[\log{c(\mathbf{x},\mathbf{y})}]
\end{aligned}
\label{E2}
\end{equation}
%使用prior的结果
When this prior is a diffusion model with latent variable $x_1,...,x_T$, and the approximate variational posterior $q(x)$ is defined as point estimate $q(\mathbf{x})=\delta(\mathbf{x}-\eta)$ \cite{graikos2022diffusion}, this optimization become:
\begin{equation}
\small
\begin{aligned}
F = \sum_t\mathbb{E}_{\epsilon\sim \mathcal{N}(0,I)}[\left \Vert \epsilon - \epsilon_{\theta}(\mathbf{x_t},t) \right \Vert^2_2] -\mathbb{E}_{q(\mathbf{x})}[\log{c(\mathbf{\eta},\mathbf{y})}] \\ \mathbf{x}_t= \sqrt{\bar{\alpha}_t}\eta + \sqrt{1-\bar{\alpha}_t}\epsilon
\end{aligned}
\label{E5}
\end{equation}
This equation optimizes $\eta$ which has the same dimensionality as data. We can regard this equation as sampling pixels using diffusion models to satisfy the constraint given condition $y$.

Especially, when constraints $c(\mathbf{x},\mathbf{y})$ is a hard and non-differentiable constraint, say a deterministic function $x=f(y)$. 
Then the gradient descent steps will be performed with respect to $\mathbf{y}$ on
\begin{equation}
\small
\begin{aligned}
\sum_t\mathbb{E}_{\epsilon\sim \mathcal{N}(0,I)}[\left \Vert \epsilon - \epsilon_{\theta}(\sqrt{\bar{\alpha}_t}f(\mathbf{y}) + \sqrt{1-\bar{\alpha}_t}\epsilon,t) \right \Vert^2_2]
\end{aligned}
\label{E6}
\end{equation}
Since image $x$ is determined by $y$, we can regard this equation as sampling $y$ instead of directly sampling pixels using diffusion models.
When we involve techniques of differentiable image parameterization, $y$ becomes the parameters of a network, $f$ becomes a differentiable generator, and it transforms parameters $\mathbf{y}$ to create an image $\mathbf{x} = f(y)$. 
For example, \cite{poole2022dreamfusion} define $y$ as parameters of a NERF and generate a 3D object using a 2D diffusion prior.

\subsection{Our method - Image Editing Paradigm}
% Our work is different from this definition in two aspects.
Although this method has had good results, there are two essential points that have not been fully discussed - optimization target and step-pruning strategy.
In this section, we will first discuss the choice of optimization target and then introduce our step-pruning strategy in the next section.

Different from sampling pixels $\eta$ or latent variable $y$, we aim to explore a new paradigm of using diffusion prior, where we use equation \eqref{E6} to optimize parameters $\phi$ of a differentiable generator $f_\phi$. 
\begin{equation}
\small
\begin{aligned}
\min_{\phi}\sum_t\mathbb{E}_{\epsilon\sim \mathcal{N}(0,I)}[\left \Vert \epsilon - \epsilon_{\theta}(\sqrt{\bar{\alpha}_t}f_\phi(\mathbf{y}) + \sqrt{1-\bar{\alpha}_t}\epsilon,t) \right \Vert^2_2]
\end{aligned}
\label{E8}
\end{equation}
We can regard this as optimizing a translation, after which images will change toward the mode defined by the text description of the multi-modal diffusion model.
For example, $y$ is the input image, $f$ is an image-to-image translation network, and the output image $x$ is sampled from the mode by indirectly optimizing the $f_\phi$.

% 放一张训练框架的图

This paradigm benefits us from three aspects. 

% 1 解决了采样pixel的问题
% 即使在图像生成任务中，这里我们不需要考虑t，因为理论上所有整个t对生成任务都会有作用。但优化pixels的方法仍旧不好，通常会出现一些loss，因此需要我们的后处理。
% 原因是 pixel space的性质并不好，而allow us to express constraints, optimize in more compact spaces (e.g., arbitrary resolution coordinate-based MLPs), or leverage more powerful optimization algorithms for traversing pixel space.
% 1) Sampling pixels $\eta$, we notice that the generated samples x, although having converged towards a correct mode of p(x), still exhibit a noticeable amount of noise.
% Using the parameterization techniques allows us to express constraints, optimize in more compact spaces, or leverage more powerful optimization algorithms for traversing pixel space.
1) It can produce higher-quality results than sampling pixels $\eta$ with some constraints on image condition $y$. 
Even in the image generation task, where all steps make a contribution and results are not susceptible to the choice of steps, sampling pixels $\eta$ still exhibit low-quality problems. 
Using parametric techniques allows us to express constraints, optimize in a more compact space, or take advantage of more powerful optimization algorithms to traverse the pixel space.
% 在image editing任务中，不同于类别标签，图像是一种很强的条件，我们需要保留其较多的信息，因此使用differentiable f，将其作为网络的输入是一种更优的做法
Unlike category labels, images are vital in editing tasks, and we need to utilize and retain more of their information. 
Therefore, we used the form of hard constraint, making the original image the input of $f_\phi$.

% 2 即使optimize network更耗时间，但是有更好的规模性，并且只需要一次forward，摆脱了non-iterative的问题
% 深层次原因是相同translation在同一domain中有着很强的共性，因此我们不需要做很多重复的计算，而通过网络去学习
2) It also demonstrates scalability, though optimizing the network usually requires more time and computation resources. 
Once the network is optimized, we only need one forward to finish image editing. 
Besides, it is easy to generalize for other images in the same domain because the exact semantic translation has a strong commonality in the same domain. 
For example, when we do expression transformations such as happy in the face domain, the semantic information that needs to be modified for all faces is consistent. 
Therefore, we can generalize our trained network for images in the same domain.

% 3 支持我们解决step-pruning的问题
3) It allows and facilitates our step-pruning strategy.
The origin paradigm requires us to compute for all $t$ in each optimization iteration,  
but it isn't easy to guide the sample towards a mode in image generation applications\cite{graikos2022diffusion}.
Existing works either anneal $t$ from high values to low values \cite{graikos2022diffusion} or randomly pick $t$ \cite{poole2022dreamfusion}, but these strategies still fall short of image editing requirements. 

\subsection{Our method - Entropy-based step-pruning strategy}

% 根据语义变化将生成过程拆分成不同阶段是一个非常重要的课题，尤其对于image editing来说
Disassembling the generation process according to semantics is a critical topic. 
Generative models with hierarchy properties have been discussed in detail.
For example, it has been shown that different StyleGAN layers are responsible for different levels of detail in the generated image.
% diffusion model中关于该问题的讨论还不够深刻
However, it is still an open problem what information the diffusion models learn at each noise level during training. 
% 一些初步讨论
Some researchers try to interpret this problem from the perspective of pretext task - denoise.
They categorize the process into coarse, content, and clean-up three stages according to the perceptual distance\cite{choi2022perception}.

% 这样的划分过于笼统，在编辑过程中，实际上更加复杂，使用该划分并不能满足要求
We found that the actual situation is much more complicated in the editing task.
% 不同编辑使用不同t有效果的例子，side view的例子

As illustrated in Fig, xxxx
Even steps in the clean-up stage can modify the global structure of an image.


% 我们采取一种更加直接的方式进行分析

Given the original image $\mathbf{y}$, we compute the gradient of the image at the time step $t$ with diffusion models conditioned on the specific textual description $\gamma$. 
\begin{eqnarray}
d = \nabla_{\mathbf{y}}\left \Vert \epsilon - \epsilon_{\theta}(\sqrt{\bar{\alpha}_t}\mathbf{y} + \sqrt{1-\bar{\alpha}_t}\epsilon,t,\gamma) \right \Vert^2_2
\end{eqnarray}
In the following description, we omit this symbol $\gamma$ for brevity. 

The gradient represents the direction in which the input image $y$ should move to the target mode at the timestep $t$.
We first convert the gradient to a confidence score through the softmax operation.
% 跟一句解释, confidence越大的方向，表明当前时刻网络认为该图片朝着target mode必需的变化量
\begin{eqnarray}
p_i = \sigma(d_i) = \frac{e^{d_{i}}}{\sum_{j=1} e^{d_{j}}} \ \ \ for\ i=1,2,\dots,H \cdot W \cdot C
\end{eqnarray}
where $d_i$ is the $i$th value of the flattened gradient map.
The larger the confidence score, the more necessary the gradient is as the image moves toward the target mode.
% entropy代表，这个t包含这样的方向程度，包含的这样方向越多，这个t对move to target mode的贡献就越大
To evaluate the entire confidence map, we calculated its entropy:
\begin{equation}
\small
\begin{aligned}
\mathcal{H}(p)=-\sum_{i}p_i\log p_i
\end{aligned}
\label{E7}
\end{equation}
The intuition is that the smaller the entropy, the more the gradient map is composed of values with high confidence. The less cluttered the entire gradient, the more helpful information it contains, and therefore the more important it is.

We have empirically observed in our experiments that it is indeed a better metric.

% 结合图的叙述
It's also useful for recognizing t=200 in side view well and has effects in other edits too. This metric can find practical steps for most editing.

Based on this, we propose a step-pruning strategy. 
Before training our image editing network, we compute the expectation of confidence entropy of all original images $\mathbf{y} \sim q(\mathbf{y})$ for each time step $t$ and ignore $t$ whose value falls below a threshold $\xi$. 

This parameter can be used to control the tolerance for uncorrelated $t$. 
When some semantics involves more steps to change, using a smaller $\xi$ will cause the most relevant features to change, but the semantics of the change is relatively simple.
Using a larger $\xi$ can be edited more comprehensively, but it's easy to introduce uncorrelated $t$.
% 在每一个编辑之前，我们计算他们针对editing的confidence entropy，设定一个threshold值选取其中较小的time step，然后在训练时只采相应的t
Training our image editing network $f_\phi$ with this strategy is shown in Alg. \ref{alg:cap}. 

\begin{algorithm}
\caption{training with step-pruning strategy}\label{alg:cap}
\begin{algorithmic}
\State $ S = \emptyset $
\For{$t = T,...,1 $}
    \State $e = \mathbb{E}_{\mathbf{y}}[\mathcal{H}(\sigma(\nabla_{\mathbf{y}}\left \Vert \epsilon - \epsilon_{\theta}(\sqrt{\bar{\alpha}_t}\mathbf{y} + \sqrt{1-\bar{\alpha}_t}\epsilon,t) \right \Vert^2_2))$]
    \If{$e < \xi$}
        \State $S=S \cup t$
    \EndIf
\EndFor
\Repeat
    \State $\mathbf{y} \sim q(\mathbf{y})$
    \State $t \sim S$ 
    \State $\epsilon \sim \mathcal{N}(0,I)$
    \State Take gradient descent step on 
    \State $\qquad \nabla_{\phi}\left \Vert \epsilon - \epsilon_{\theta}(\sqrt{\bar{\alpha}_t}f_\phi(\mathbf{y}) + \sqrt{1-\bar{\alpha}_t}\epsilon,t) \right \Vert^2_2$
\Until converged
\end{algorithmic}
\end{algorithm}







==> legacy/04_method_v3.tex <==
\section{Method}
\label{sec:method}
%%%% background: diffusion model as plug-and-play prior

\subsection{Our method - Image Editing Paradigm}
% Our work is different from this definition in two aspects.
Although this method has had good results, two essential points have not been fully discussed - optimization target and step-pruning strategy.
In this section, we will first discuss the choice of optimization target and then introduce our step-pruning strategy in the next section.

Both sampling pixels $\eta$ \cite{graikos2022diffusion} and optimizing latent variable $\mathbf{y}$\cite{poole2022dreamfusion} assume the constraint $c(\mathbf{x}, \mathbf{y})$ is pre-defined.
In this work, we consider a new scenario where the constraint is unknown and propose our new paradigm of image editing with diffusion models. 

We hope to derive an appropriate constraint $c(\mathbf{x]}, \mathbf{y})$ through the condition $mathbf{y}$ and a diffusion model $p_\theta$.
Specifically, we define this hard constraint $c(\mathbf{x},\mathbf{y})$ as an image editing network $f$ with parameters $\phi$, condition $y$ as the input image in the source domain. We can compute the output image via $\mathbf{x}=f_\phi(\mathbf{y})$. 
This constraint is common in image-to-image translation tasks, where there is a one-to-one pair relationship between each input and output image.
As shown in Fig xx, we use a multi-modal diffusion model to help learn this network with the objective below: 
\begin{equation}
\small
\begin{aligned}
\min_{\phi}\mathbb{E}_{\epsilon,t}[\left \Vert \epsilon - \epsilon_{\theta}(\sqrt{\bar{\alpha}_t}f_\phi(\mathbf{y}) + \sqrt{1-\bar{\alpha}_t}\epsilon,t,\gamma) \right \Vert^2_2]
\end{aligned}
\label{E8}
\end{equation}

Where $p_\theta$ is fixed during optimization and is conditioned on the natural language description $\gamma$ entered by the user, in the following description, we omit this symbol $\gamma$ for brevity.
This equation optimizes the $f_\phi$ so that its output image looks like a sample from the desired mode of the multi-modal diffusion model. 

This paradigm benefits us from three aspects: 
1) It can produce higher-quality results than directly sampling pixels $\eta$. 
Even in the image generation task, where all steps contribute and results are not susceptible to the choice of steps, sampling pixels $\eta$ still exhibit low-quality problems and need post-processing\cite{graikos2022diffusion}.
Using a network can extract more precise semantics from the original image and learn more relevant places for editing. 
We can also use more powerful optimization algorithms and express more constraints to train this network.


2) It also demonstrates scalability, though optimizing the network usually requires more time and computation resources. 
For example, once the network is optimized, we only need one forward to finish image editing. 
Besides, it is easy to generalize for other images in the same domain because the exact semantic translation has a strong commonality in the same domain. 
For example, when we do expression translations such as happy in the face domain, the semantic information that needs to be modified for all faces is consistent. 
Therefore, we can generalize our trained network for images in the same domain.

3) This idea of using the diffusion model as a prior instead of itself facilitate us to analyze and select key step $t$ for each editing. 
% 加一句分析？
Although the choice of step t is now flexible, the analysis is not enough.
Different from the generation task, where all steps $t$ make a contribution, the semantic changes required for editing may occur in a specific stage of the process.
Unfortunately, existing random and annealing strategies can not meet the requirements.
Therefore, we propose our step-pruning strategy.




\subsection{Our method - Entropy-based step-pruning strategy}

% 根据语义变化将生成过程拆分成不同阶段是一个非常重要的课题，尤其对于image editing来说
Disassembling the generation process according to semantics is a critical topic. 
Generative models with hierarchy properties have been discussed in detail.
For example, it has been shown that different StyleGAN layers are responsible for different levels of detail in the generated image.
% diffusion model中关于该问题的讨论还不够深刻
However, it is still an open problem what information the diffusion models learn at each noise level during training. 
% 一些初步讨论
Some researchers try to interpret this problem from the perspective of pretext task - denoise.
They categorize the process into coarse, content, and clean-up three stages according to the perceptual distance\cite{choi2022perception}.

% 这样的划分过于笼统，在编辑过程中，实际上更加复杂，使用该划分并不能满足要求
We found that the actual situation is much more complicated in the editing task.
% 不同编辑使用不同t有效果的例子，side view的例子

As illustrated in Fig, xxxx
Even steps in the clean-up stage can modify the global structure of an image.


% 我们采取一种更加直接的方式进行分析

Given the original image $\mathbf{y}$, we compute the gradient of the image at the time step $t$ with diffusion models conditioned on the specific textual description $\gamma$. 
\begin{eqnarray}
d = \nabla_{\mathbf{y}}\left \Vert \epsilon - \epsilon_{\theta}(\sqrt{\bar{\alpha}_t}\mathbf{y} + \sqrt{1-\bar{\alpha}_t}\epsilon,t,\gamma) \right \Vert^2_2
\end{eqnarray}
 
The gradient represents the direction in which the input image $y$ should move to the target mode at the timestep $t$.
We first convert the gradient to a confidence score through the softmax operation.
% 跟一句解释, confidence越大的方向，表明当前时刻网络认为该图片朝着target mode必需的变化量
\begin{eqnarray}
p_i = \sigma(d_i) = \frac{e^{d_{i}}}{\sum_{j=1} e^{d_{j}}} \ \ \ for\ i=1,2,\dots,H \cdot W \cdot C
\end{eqnarray}
where $d_i$ is the $i$th value of the flattened gradient map.
The larger the confidence score, the more necessary the gradient is as the image moves toward the target mode.
% entropy代表，这个t包含这样的方向程度，包含的这样方向越多，这个t对move to target mode的贡献就越大
To evaluate the entire confidence map, we calculated its entropy:
\begin{equation}
\small
\begin{aligned}
e=\mathcal{H}(p)=-\sum_{i}p_i\log p_i
\end{aligned}
\label{E7}
\end{equation}
The intuition is that the smaller the entropy, the more the gradient map is composed of values with high confidence. The less cluttered the entire gradient, the more helpful information it contains, and therefore the more important it is.

We write these two steps into function $m(\dot)$ :
\begin{equation}
\small
\begin{aligned}
e = m(d)
\end{aligned}
\label{E7}
\end{equation}

We have empirically observed in our experiments that it is indeed a better metric.

% 结合图的叙述
It's also useful for recognizing t=200 in side view well and has effects in other edits too. This metric can find practical steps for most editing.

Based on this, we propose a step-pruning strategy. 
Before training our image editing network, we compute the expectation of confidence entropy of all original images $\mathbf{y} \sim q(\mathbf{y})$ for each time step $t$ and ignore $t$ whose value falls below a threshold $\xi$. 

This parameter can be used to control the tolerance for uncorrelated $t$. 
When some semantics involves more steps to change, using a smaller $\xi$ will cause the most relevant features to change, but the semantics of the change is relatively simple.
Using a larger $\xi$ can be edited more comprehensively, but it's easy to introduce uncorrelated $t$.
% 在每一个编辑之前，我们计算他们针对editing的confidence entropy，设定一个threshold值选取其中较小的time step，然后在训练时只采相应的t
Training our image editing network $f_\phi$ with this strategy is shown in Alg. \ref{alg:cap}. 

\begin{algorithm}
\caption{training with step-pruning strategy}\label{alg:cap}
\begin{algorithmic}
\State $ S = \emptyset $
\For{$t = T,...,1 $}
    % \State $e = \mathbb{E}_{\mathbf{y}}[\mathcal{H}(\sigma(\nabla_{\mathbf{y}}\left \Vert \epsilon - \epsilon_{\theta}(\sqrt{\bar{\alpha}_t}\mathbf{y} + \sqrt{1-\bar{\alpha}_t}\epsilon,t) \right \Vert^2_2))]$
    \State $e = \mathbb{E}_{\mathbf{y}}[m(\nabla_{\mathbf{y}}\left \Vert \epsilon - \epsilon_{\theta}(\sqrt{\bar{\alpha}_t}\mathbf{y} + \sqrt{1-\bar{\alpha}_t}\epsilon,t) \right \Vert^2_2)]$
    \If{$e < \xi$}
        \State $S=S \cup t$
    \EndIf
\EndFor
\Repeat
    \State $\mathbf{y} \sim q(\mathbf{y})$
    \State $t \sim S$ 
    \State $\epsilon \sim \mathcal{N}(0,I)$
    \State Take gradient descent step on 
    \State $\qquad \nabla_{\phi}\left \Vert \epsilon - \epsilon_{\theta}(\sqrt{\bar{\alpha}_t}f_\phi(\mathbf{y}) + \sqrt{1-\bar{\alpha}_t}\epsilon,t) \right \Vert^2_2$
\Until converged
\end{algorithmic}
\end{algorithm}


\subsection{Implementation details}
\textbf{StyleGAN Mapper}

\textbf{Adaptor}


==> legacy/04_method_v4.tex <==
\section{Method}
\label{sec:method}
\subsection{Image manipultaion paradigm}

\begin{figure*}[htbp]
    \centering
    \includegraphics[width=18cm]{figs/framework.pdf}
    \caption{General framework of our method. \textbf{Top}: the entropy-based step pruning strategy. \textbf{Bottom}: Using the selected timesteps and the pretrain diffusion model $p_\theta$ to train the image manipulator $f_\phi$}.
    \label{framework}
\end{figure*}


According to the above formulations, our image manipulator can also be a hard image-conditional model, i.e., $x=f(y)$, where $y$ is an input image and $f()$ is usually a CNN network that outputs an edited image $x$. 
We expect our image manipulator can not only utilize rich guidance from text-to-image diffusion models but also implement text-driven editing without the diffusion model directly participating.

% 我们讨论一种新的情况，这里f是可优化的
Motivated by this, we are exploring a paradigm different from existing discussions about diffusion prior, where $f()$ becomes the  optimization target. 
It means we use equation \eqref{E9} to optimize parameters $\phi$ of our image manipulator $f_\phi$ as shown in Fig.\ref{framework}. 
\begin{equation}
\small
\begin{aligned}
\min_{\phi}\mathbb{E}_{\epsilon,t}[\left \Vert \epsilon - \epsilon_{\theta}(\sqrt{\bar{\alpha}_t}f_\phi(y) + \sqrt{1-\bar{\alpha}_t}\epsilon,t) \right \Vert^2_2].
\end{aligned}
\label{E10}
\end{equation}
We can regard this optimization process as ``sampling" an image translation direction. 
With this direction, the image will change toward the target mode of diffusion models.


\begin{figure}[htbp]
    \centering
    \includegraphics[width=8cm]{figs/optimize_choice.pdf}
    \caption{The advantages of optimizing the network, and the editing prompt is ``angry''. \textbf{Top}: Input image. \textbf{Middle}: Directly optimizing input image with diffusion guidance and there is a lot of small noise on the results. \textbf{Bottom} Optimizing our image manipulator with diffusion guidance. It not only guarantees the quality of the results but also edits the correct semantics.}
    \label{optimize-choice}
\end{figure}

This paradigm benefits us from two aspects. 
% 比直接优化pixel效果好
1) It can produce higher-quality results.
% 直接优化pixel本身
The most straightforward approach to seeking an image modification is to set $f()$ as the identity function, e.g., $x=y$, and then directly optimize the input image $y$.
% 直接优化不好
However, traversing pixel space often leads to bad results \cite{graikos2022diffusion}.
It is difficult to ensure the fidelity of the image because the image contains a lot of semantically irrelevant information (e.g., imperceptible information)
This information can be easily modified during this optimization process, as shown in Fig. \ref{optimize-choice}
% 优化网络让我们关注在语义信息上，同时可以用更加丰富的策略很更多的限制
Using neural networks allows us to focus only on the semantic level and we are allowed to use more powerful optimization algorithms and express more constraints to train this network.

% 比直接优化pixel效率高
2) It also demonstrates scalability, though optimizing the network usually requires more time and computation resources. 
Firstly, once the network is optimized, we only need one forward to finish image manipulation. 
Besides, it is easy to generalize for other images in the same domain because the same semantic translation has a strong commonality in the same domain.
For example, when we do expression transformations such as happiness in the face domain, the semantic information that needs to be modified for all faces is consistent. 
Therefore, we can save the overhead of generalizing this network to more images. We will discuss this quantitatively in the experimental section.

This is a win-win situation, as we take advantage of the rich patterns of the text-to-image diffusion model and the ability to easily obtain target pattern samples from text, while using a small conditional model to get rid of the large amount of computation required when inferencing with the diffusion model.


\subsection{Hybrid Quality Score(HQS)-based step selection strategy}

% 发现训练过程中，对不同的编辑，t的选取非常重要
Recalling that computing Eq. \eqref{E9} requires a time step $t$ as input, we empirically observed that the optimization of our image manipulator is susceptible to the choice of the time step $t$, as shown in Fig. \ref{t-observation}. 
Training with an inappropriate timestep has no effect while using an accurate timestep has the most obvious effect under the same iterations of optimization. 

% 这种现象是合理的，因为diffusion generation process不同阶段对应着不同的visual concept
This phenomenon is reasonable because the generation process of diffusion models can be divided into different stages corresponding to visual concepts \cite{choi2022perception}, such as the coarse, content, and clean-up stage.
Such a division is still too general and requires human intuition to first divide editing into three stages.
Therefore, we need further discussion to solve this problem.

% 定义问题 - 将接下来的讨论与image manipulator具体是什么给划分开，
The problem is defined as given an image, we expect to identify at which timestep the diffusion model contributes the most to translate the image into a target sample. 
We start our analysis with the gradients that the diffusion model provides to the image. We input the image $y$ into the diffusion model conditioned on textual description $\gamma$ at every time step $t=T,...,1$, and then compute the gradient of the image using diffusion training loss:
\begin{eqnarray}
\nabla_{y}\left \Vert \epsilon - \epsilon_{\theta}(\sqrt{\bar{\alpha}_t}y + \sqrt{1-\bar{\alpha}_t}\epsilon,t,\gamma) \right \Vert^2_2
\label{E11}
\end{eqnarray}
Since the diffusion model is fixed, we replace this result with $d(y,t,\gamma)$ for brevity.
The gradient $d(y,t,\gamma)$ represents the direction in which the input image $y$ should move to the target mode $\gamma$ at the timestep $t$.
We assume if a timestep $t$ is more important, its direction $d$ should be of higher quality than other timesteps.

To measure its quality, we have empirically observed that treating this gradient as a confidence map and computing its entropy gives us a good metric.
We first convert $d$ into a confidence score map $p$ through the softmax operation.
% 跟一句解释, confidence越大的方向，表明当前时刻网络认为该图片朝着target mode必需的变化量
\begin{eqnarray}
p_i = \sigma(d_i) = \frac{e^{d_{i}}}{\sum_{j=1} e^{d_{j}}} \ \ \ {\rm for}\ i=1,2,\dots,H \cdot W \cdot C
\label{E12}
\end{eqnarray}
where $d_i$ is the $i$th value of the flattened gradient map.
For each score of the confidence map, it represents the degree of necessity of the corresponding gradient when modifying the image. 
Next, for the whole confidence map, we calculated its entropy:
\begin{equation}
\small
\begin{aligned}
\mathcal{H}(p)=-\sum_{i}p_i\log p_i
\end{aligned}
\label{E13}
\end{equation}
The intuition is that the lower the entropy, the more the $d(y, t,\gamma)$ contains the necessary gradient, so the $t$ is more important.
This metric is susceptible to some extreme cases, such as when only a very small part of the gradient map has value. 
Such a situation will result in a very high value of our metric, but the gradient actually makes little contribution to the image.
Therefore, we introduce the L1 norm of the gradient $d(y, t,\gamma)$ to avoid this situation.
We simply negate the entropy, scale the negative entropy and L1 norm to the same order of magnitude, and add them together.
We name this metric hybrid quality score (HQS) and represent it with function $m()$ for brevity.
As shown in Fig. \ref{optimize-choice}, training with the timestep that has the higher hybrid quality score gives us the best editing results. 

% We also replace the computation process with function $m()$ for brevity, so that $e = m(d(\mathbf{y}, t,\gamma))$

\begin{figure}[htbp]
    \centering
    \includegraphics[width=8cm]{figs/HQS-v2.pdf}
    \caption{\textbf{Effect of our Hybrid Quality Score(HQS)}. \textbf{Left}: The curve of HQS at different timesteps when the prompt is ``angry". \textbf{Right}: Gradient visualization of the corresponding timestep and editing results of training our image manipulator using only this timestep.}
    \label{HQS}
\end{figure}



Based on this, we propose a step selection strategy:
Before training our image manipulator, we compute the expectation of $m(d(y, t, \gamma))$ for original images $y \sim q(y)$ at each time step $t$.
Then we ignore $t$ whose value falls below a threshold $\xi$. This parameter $\xi$ can be used to control the tolerance for uncorrelated $t$. 
When some semantics involves more steps to change, using a smaller $\xi$ will cause the most relevant features to change, but the semantics of the change is relatively simple.
% 阈值越小，就只集中使用特定的一步，那一步最为重要，但semantics就比较单一，不够自然
When we use a smaller $\xi$, only the most relevant features will change. This leads to a faster change but the semantics of the change will be relatively simple. Thus the edited image may not be natural. 
Using a larger $\xi$ makes our editing more comprehensive, but it's easy to introduce uncorrelated $t$.
So after the prompt is chosen, we first calculate the hybrid quality score of the image gradient and then set a threshold to select the desired timestep.
Training our image manipulator $f_\phi$ with this strategy is shown in Alg. \ref{alg:cap}. 

\begin{algorithm}
\caption{training with entropy-based step pruning strategy}\label{alg:cap}
\begin{algorithmic}
\State $ S = \emptyset $
\For{$t = T,...,1 $}
    % 使用SUM
    \State $e = \mathbb{E}_{y}[HQS(\nabla_{y}\left \Vert \epsilon - \epsilon_{\theta}(\sqrt{\bar{\alpha}_t}y + \sqrt{1-\bar{\alpha}_t}\epsilon,t) \right \Vert^2_2)$]
    \If{$e > \xi$}
        \State $S=S \cup t$
    \EndIf
\EndFor
\Repeat
    % q0
    \State $y \sim q(y)$
    \State $t \sim S$ 
    \State $\epsilon \sim \mathcal{N}(0,I)$
    \State Take gradient descent step on 
    \State $\qquad \nabla_{\phi}\left \Vert \epsilon - \epsilon_{\theta}(\sqrt{\bar{\alpha}_t}f_\phi(y) + \sqrt{1-\bar{\alpha}_t}\epsilon,t) \right \Vert^2_2$
\Until converged
\end{algorithmic}
\end{algorithm}
Such a strategy is proven effective in our experiments, and the above analysis is agnostic to the form of our image manipulator, so it can be extended to any image editing framework. 

==> legacy/04_method_v5.tex <==
\section{Method}
\label{sec:method}
\subsection{Distilling the diffusion model}
\label{distilling-the-diffusion-model}
\begin{figure*}[htbp]
    \centering
    \includegraphics[width=17cm]{figs/framework.pdf}
    \caption{ \textbf{General framework of Selective Diffusion Distillation (SDD)}. \textbf{Top}: HQS-based step selection strategy. \textbf{Bottom}: Using the selected timesteps and the pretrain diffusion model $p_\theta$ to train the image manipulator $f_\phi$.}
    \label{framework}
\end{figure*}

% 3.2讲如何使用diffusion as prior
% 1 如何使用diffusion as prior
%。  optimize random t goes here.
%  优化x的公式放在这
% 2 hard constrain下的形式，仅当x=f(y)，c(x,y)=1，else = 0, indicator function
% 3 dreamfusion就是一种hard consrtain
%  公式放在这
%  做法，优化y, 加粗

% 我们目的是啥
Our goal is to take the diffusion model as a teacher model to train a lightweight image manipulator.
% 我们做了啥
We first define our problem according to the definition in Sec. \ref{Diffusion-models-as-prior}. 
Training the image manipulator with diffusion prior can also be categorized as an optimization problem with a hard constraint. In this situation, the hard constraint f(y) becomes the image manipulator. The difference between our formulation and the previous formulation is the optimized target. We use equation \eqref{E10} to optimize parameters $\phi$ of our image manipulator $f_\phi$ as shown in Fig. \ref{framework}. 

\begin{equation}
\small
\begin{aligned}
\min_{\phi}\mathbb{E}_{\epsilon,t}[\left \Vert \epsilon - \epsilon_{\theta}(\sqrt{\bar{\alpha}_t}f_\phi(y) + \sqrt{1-\bar{\alpha}_t}\epsilon,t) \right \Vert^2_2].
\end{aligned}
\label{E10}
\end{equation}

% 没懂
We can regard this optimization process as ``sampling" an image translation direction. 
With this direction, the image will change toward the target mode of diffusion models.

This paradigm benefits us from two aspects. 
% 比使用diffusion process要好
Firstly, once the network is optimized, we only need to perform the fast image manipulation through one forward, and the diffusion model is no more required. By using diffusion as a teacher model, we distill the heavy denoising process into a single inference of our network. Not to mention that the manipulator network itself is lighter than the U-net of the diffusion model.
% 比使用diffusion process效率高
Secondly, our network also demonstrates scalability. 
Though optimizing the network usually requires more time and computation resources, it is still worthwhile since the network is easy to generalize to other images in the same domain. 
We find that there is strong common knowledge when translating images in the same domain to a specific semantic direction. Simply reusing the network also works well for all images in the pretrain image domain.
For example, when we do facial expression transformations such as happiness, the semantic information that needs to be modified for all faces is similar. In this case, we do not retrain the network.
Therefore, we save the overhead when manipulating more images. We will discuss this quantitatively in Sec. \ref{quality-efficient-exp}.

This is a win-win situation, as we take advantage of the rich patterns of the text-to-image diffusion model and the ability to easily obtain target pattern samples from text, while using a small conditional model to get rid of a large amount of computation required when inference with the diffusion model.


\subsection{Selecting timestep with the Hybrid Quality Score (HQS)}

\begin{figure}[htbp]
    \centering
    \includegraphics[width=8cm]{figs/t_observation.pdf}
    \caption{ \textbf{Results of different manipulations using different timestep}. Better results for each manipulation are highlighted with red boxes. For one manipulation, different time steps show different effects. For different manipulations, different time steps achieve the best performance.}
    \label{t-observation}
\end{figure}

% 发现训练过程中，对不同的编辑，t的选取非常重要
Recalling that computing Eq. \eqref{E10} requires a timestep $t$ as input, we empirically observed that the optimization of our image manipulator is susceptible to the choice of the timestep $t$, as shown in Fig. \ref{t-observation}. 
Training with an inappropriate timestep has no effect while using an accurate timestep has the most obvious effect under the same iterations of optimization. 

% 这种现象是合理的，因为diffusion generation process不同阶段对应着不同的visual concept
This phenomenon is reasonable because the generation process of diffusion models can be divided into different stages corresponding to visual concepts \cite{choi2022perception}, such as the coarse, content, and clean-up stage.
Such a division is still too general and requires human intuition to divide the process into three stages.
Therefore, we need further discussions on this problem.

% 定义问题 - 将接下来的讨论与image manipulator具体是什么给划分开，
The problem is defined as given an image, we expect to identify at which timestep the diffusion model contributes the most to translate the image into a target distribution. 
We start our analysis with the gradients that the diffusion model provides to the image. We input the image $y$ into the diffusion model conditioned on textual description $\gamma$ at every timestep $t\in\{T,\cdots,1\}$, and then compute the gradient of the image using diffusion training loss:
\begin{eqnarray}
d_t(y,\gamma) = \nabla_{y}\left \Vert \epsilon - \epsilon_{\theta}(\sqrt{\bar{\alpha}_t}y + \sqrt{1-\bar{\alpha}_t}\epsilon,t,\gamma) \right \Vert^2_2,
\label{grad}
\end{eqnarray}
where $d_t(y,\gamma) \in \mathbb{R}^{1\times H\cdot W\cdot C}$ represents the direction in which the input image $y$ should move to the target distribution $\gamma$ at the timestep $t$.
We assume if a timestep $t$ is more important, its direction $d$ should be of higher quality than other timesteps.

To measure its quality, we have empirically observed that treating this gradient as a confidence map and computing its entropy gives us a good metric.
We first convert $d_t$ into a confidence score map $p_t$ through the softmax operation.
% 跟一句解释, confidence越大的方向，表明当前时刻网络认为该图片朝着target mode必需的变化量
% \begin{eqnarray}
% p_t = \mathrm{softmax}(d_t)
% \label{E12}
% \end{eqnarray}

For each score of the confidence map, it represents the degree of necessity of the corresponding gradient when modifying the image. 
Next, for the whole confidence map, we calculated its entropy:
\begin{equation}
% \small
% \begin{aligned}
H_t = -\sum_{i}p^i_t \log p^i_t,
% \end{aligned}
\label{E13}
\end{equation}
where $p_t^i$ is the i-th element of $p_t$.

The intuition is that the lower the entropy, the more the $d_t(y,\gamma)$ contains the necessary gradient, so the $t$ is more important.
Then, we found this metric is susceptible to some extreme cases, such as when only a very small part of the gradient map has value. 
This will result in a very high value of $H_t$, but the gradient actually makes little contribution to the image.
Therefore, we introduce the $L_1$ norm of the gradient $d_t(y,\gamma)$ to avoid this situation:
\begin{equation}
% \small
% \begin{aligned}
N_t = \sum_{i} |d_t^i|,
% \end{aligned}
\label{E14}
\end{equation}
where $d_t^i$ is the i-th element of $d_t$.
This metric ensures the magnitude of the overall information of the gradient, thereby avoiding the misjudgment of the entropy metric caused by the local large value.
To combine the two metrics, we first transform $H = [H_1,\cdots, H_T]$ to $\bar{H} = [\bar{H}_1,\cdots,\bar{H}_T]$ by using min-max normalization as follows:
\begin{equation}
% \small
% \begin{aligned}
\bar{H}_t = \frac{H_t - \mathrm{min}(H)}{\mathrm{max}(H) - \mathrm{min}(H)},
% \end{aligned}
\label{E15}
\end{equation}
and we also do the same to $N$ to get $\bar{N}$.

Significantly, given manipulation target $\gamma$, we consider timestep $t$ with lower $\bar{H}_t$ and higher $\bar{N}_t$ to be optimal, so we define a metric called Hybrid Quality Score (HQS) :
\begin{equation}
\mathrm{HQS}(\gamma) = \mathbb{E}_{y}[\bar{N} - \bar{H}],
\label{eq:HQS}
\end{equation}
Where $HQS \in \mathbb{R}^{1 \times T}$.
As shown in Fig. \ref{HQS}, training with the timestep that has the higher hybrid quality score gives us rich semantic gradients\footnote{we clip and normalize the gradient value for better illustration.} and better editing results. 

% We also replace the computation process with function $m()$ for brevity, so that $e = m(d(\mathbf{y}, t,\gamma))$

\begin{figure}[htbp]
    \centering
    \includegraphics[width=8cm]{figs/HQS.pdf}
    \caption{\textbf{Effect of our Hybrid Quality Score (HQS)}. \textbf{Left}: The curve of HQS at different timesteps when the prompt is ``angry". \textbf{Right}: Gradient visualization of the corresponding timestep and editing results of training our image manipulator using only this timestep.}
    \label{HQS}
\end{figure}


Based on this, we propose a timestep selection strategy:
Before training our image manipulator, we compute the $HQS(\gamma)$ for original images $y \sim q(y)$ at each timestep $t$.
Then we ignore $t$ whose value falls below a threshold $\xi$. This parameter $\xi$ can be used to control the tolerance for uncorrelated $t$. 
% When some semantics involves more steps to change, using a smaller $\xi$ will cause the most relevant features to change, but the semantics of the change is relatively simple.
% 阈值越小，就只集中使用特定的一步，那一步最为重要，但semantics就比较单一，不够自然
When using a smaller $\xi$, only the most relevant features will change. This leads to a faster change but the semantics of the change will be relatively simple. Thus the edited image may not be natural. 
Using a larger $\xi$ makes our editing more comprehensive, but it's easy to introduce uncorrelated $t$.
So after the prompt is chosen, we first calculate the hybrid quality score of the image gradient and then set a threshold to select the desired timestep.
Training our image manipulator $f_\phi$ with this strategy is shown in Alg. \ref{alg:cap}. 

\begin{algorithm}
\caption{Selective Diffusion Distillation}\label{alg:cap}
\begin{algorithmic}[1]
\State {\bfseries Input:} text prompts $\gamma$, image data $q(y)$, threshold $\xi$, 
 pretrained diffusion model $\epsilon_{\theta}$
\State Compute $\mathrm{HQS}(\gamma)$ by Eq. \eqref{eq:HQS}
\State $S=\{t \mid \mathrm{HQS}_t > \xi \}$
\State Randomly initialize our image manipulator $f_\phi$
\Repeat
    % q0
    \State $y \sim q(y)$, $t \in S$, $\epsilon \sim \mathcal{N}(\mathbf{0},\mathbf{I})$
    \State Take gradient descent step on 
    \State $\qquad \nabla_{\phi}\left \Vert \epsilon - \epsilon_{\theta}(\sqrt{\bar{\alpha}_t}f_\phi(y) + \sqrt{1-\bar{\alpha}_t}\epsilon,t) \right \Vert^2_2$
\Until converged
\end{algorithmic}
\end{algorithm}

Using this strategy leads to a set $S$ of a smaller size. This selected $S$ contains more effective timesteps than the whole timesteps set. Training the image manipulator with selected $S$ finally contributes to faster convergence speed.
We prove the effectiveness in the Sec. \ref{step-selection-exp}. The above analysis is agnostic to the form of our image manipulator, so it can be extended to any image manipulation framework. 

==> legacy/04_method_v6.tex <==
\section{Method}
\label{sec:method}
\subsection{Learning image manipulator with Diffusion Models}
\label{distilling-the-diffusion-model}
\begin{figure*}[htbp]
    \centering
    \includegraphics[width=17cm]{figs/framework.pdf}
    \caption{ \textbf{General framework of Selective Diffusion Distillation (SDD)}. \textbf{Top}: HQS-based step selection strategy. \textbf{Bottom}: Using the selected timesteps and the pretrain diffusion model $p_\theta$ to train the image manipulator $f_\phi$.}
    \label{framework}
\end{figure*}

% 3.2讲如何使用diffusion as prior
% 1 如何使用diffusion as prior
%。  optimize random t goes here.
%  优化x的公式放在这
% 2 hard constrain下的形式，仅当x=f(y)，c(x,y)=1，else = 0, indicator function
% 3 dreamfusion就是一种hard constrain
%  公式放在这
%  做法，优化y, 加粗

% 我们目的是啥
We aim to take the diffusion model as a source of semantic guidance to train a lightweight image manipulator.
% 我们做了啥
We first define our problem according to the definition in Sec. \ref{Diffusion-models-as-prior}. 
Training the image manipulator with diffusion prior can also be categorized as an optimization problem with a hard constraint. The hard constraint f(y) becomes the image manipulator in this situation. The difference between our formulation and the previous formulation is the optimized target. We use equation \eqref{E10} to optimize parameters $\phi$ of our image manipulator $f_\phi$ as shown in Fig. \ref{framework}. 

\begin{equation}
\small
\begin{aligned}
\min_{\phi}\mathbb{E}_{\epsilon,t}[\left \Vert \epsilon - \epsilon_{\theta}(\sqrt{\bar{\alpha}_t}f_\phi(y) + \sqrt{1-\bar{\alpha}_t}\epsilon,t) \right \Vert^2_2].
\end{aligned}
\label{E10}
\end{equation}
% intuition讲下原理？
When optimizing this equation, we follow the approach of skipping the U-Net Jacobian in \cite{poole2022dreamfusion}. The gradient after skipping is equivalent to the noise predicted at the current timestep (based on the diffusion model) minus a random noise. 
According to the relationship between diffusion models and score-based models\cite{song2019score1,song2020score2}, this predicted noise from the diffusion model contains the direction from the current distribution to the target distribution.
Therefore, we can consider optimizing this equation as guiding our image manipulator by the diffusion model to output results in the target distribution.

This paradigm benefits us from three aspects.
% 解决了trade-off的问题
Firstly, regardless of the semantics learned from the diffusion model, we can always ensure the fidelity of the image manipulator by imposing regularization terms.
For instance, we want to manipulate the semantics corresponded to the early stage of diffusion models. During this stage, the diffusion model perceives limited information from the original image, resulting in a gradient with high uncertainty. If we directly manipulate images using the diffusion model, it can easily cause significant changes to the original image. However, using regularization terms, we can extract only the most relevant information from the gradient for our image manipulator.

% 编辑时更效率
Secondly, after optimizing the image manipulator, we can perform fast image manipulation through a single forward pass without requiring the diffusion model. Moreover, the manipulator network is lighter than the U-net in the diffusion model.
Furthermore, as described in Sec.~\ref{sec:experiments}, we only need to optimize a 4-layer MLP model when using a pre-trained model. This significantly reduces both our training and inference costs.

% 训练成本是可接受的
Thirdly, our manipulator also demonstrates scalability. 
Though optimizing the image manipulator usually requires more time and computation resources, it is still worthwhile since it is easy to generalize to other images in the same domain. 
We find common knowledge when translating images in the same domain to a specific semantic direction. Reusing the network also works well for all images in the train image domain.
For example, when we do facial expression transformations such as happiness, the semantic information that needs to be modified for all faces is similar. In this case, we do not retrain the network.
Therefore, we save the overhead when manipulating more images. We will discuss this quantitatively in Sec.~\ref{quality-efficient-exp}.



\subsection{Selecting timestep with the Hybrid Quality Score (HQS)}

\begin{figure}[htbp]
    \centering
    \includegraphics[width=8cm]{figs/t_observation.pdf}
    \caption{ \textbf{Results of different manipulations using different timestep}. Better results for each manipulation are highlighted with red boxes. For one manipulation, different time steps show different effects. For different manipulations, different time steps achieve the best performance.}
    \label{t-observation}
\end{figure}

% 训练过程中，对不同的编辑，t的选取非常重要
According to our hypothesis, the guidance provided by the diffusion model at different timesteps is different, given the same text. We also observe the optimization of the image manipulator is susceptible to the choice of the timestep $t$, as shown in Fig. \ref{t-observation}. 
Training with an inappropriate timestep has no effect, while using an accurate timestep has the most obvious effect under the same iterations of optimization. 

% 这种现象是合理的，因为diffusion generation process不同阶段对应着不同的visual concept
The previous work \cite{choi2022perception} divides the diffusion process into three stages: coarse, content, and clean-up. However, this general division may not be suitable for semantic manipulations because different semantics may require different steps for optimal results.
Therefore, we need further discussions on this problem.

% 定义问题 - 将接下来的讨论与image manipulator具体是什么给划分开，
The problem is defined as given an image, we expect to identify at which timestep the diffusion model contributes the most to translate the image into a target distribution. 
We start our analysis with the gradients the diffusion model provides to the image. We input the image $y$ into the diffusion model conditioned on textual description $\gamma$ at every timestep $t\in\{T,\cdots,1\}$, and then compute the gradient of the image using diffusion training loss:
\begin{eqnarray}
d_t(y,\gamma) = \nabla_{y}\left \Vert \epsilon - \epsilon_{\theta}(\sqrt{\bar{\alpha}_t}y + \sqrt{1-\bar{\alpha}_t}\epsilon,t,\gamma) \right \Vert^2_2,
\label{grad}
\end{eqnarray}
where $d_t(y,\gamma) \in \mathbb{R}^{1\times H\cdot W\cdot C}$ represents the direction in which the input image $y$ should move to the target distribution $\gamma$ at the timestep $t$.
If a timestep $t$ is more important, its direction $d$ should be higher quality than other timesteps.

To measure its quality, we have empirically observed that treating this gradient as a confidence map and computing its entropy gives us a good metric.
We first convert $d_t$ into a confidence score map $p_t$ through the softmax operation.
Each score of the confidence map represents the degree of necessity of the corresponding gradient when modifying the image. 
Next, for the whole confidence map, we calculated its entropy:
\begin{equation}
% \small
% \begin{aligned}
H_t = -\sum_{i}p^i_t \log p^i_t,
% \end{aligned}
\label{E13}
\end{equation}
where $p_t^i$ is the i-th element of $p_t$.
The intuition is that the lower the entropy, the more the $d_t(y,\gamma)$ contains the necessary gradient, so the $t$ is more important.
Then, we found this metric susceptible to extreme cases, such as when only a very small part of the gradient map has value. 
This will result in a very high value of $H_t$, but the gradient contributes little to the image.
Therefore, we introduce the $L_1$ norm of the gradient $d_t(y,\gamma)$ to avoid this situation:
\begin{equation}
% \small
% \begin{aligned}
N_t = \sum_{i} |d_t^i|,
% \end{aligned}
\label{E14}
\end{equation}
where $d_t^i$ is the i-th element of $d_t$.
This metric ensures the magnitude of the overall information of the gradient, thereby avoiding the misjudgment of the entropy metric caused by the local large value.
To combine the two metrics, we first transform $H = [H_1,\cdots, H_T]$ to $\bar{H} = [\bar{H}_1,\cdots,\bar{H}_T]$ by using min-max normalization as follows:
\begin{equation}
% \small
% \begin{aligned}
\bar{H}_t = \frac{H_t - \mathrm{min}(H)}{\mathrm{max}(H) - \mathrm{min}(H)},
% \end{aligned}
\label{E15}
\end{equation}
and we also do the same to $N$ to get $\bar{N}$.

Significantly, given manipulation target $\gamma$, we consider timestep $t$ with lower $\bar{H}_t$ and higher $\bar{N}_t$ to be optimal, so we define a metric called Hybrid Quality Score (HQS) :
\begin{equation}
\mathrm{HQS}(\gamma) = \mathbb{E}_{y}[\bar{N} - \bar{H}],
\label{eq:HQS}
\end{equation}
Where $HQS \in \mathbb{R}^{1 \times T}$.
As shown in Fig. \ref{HQS}, training with the timestep with the higher hybrid quality score gives us rich semantic gradients\footnote{we clip and normalize the gradient value for better illustration.} and better editing results. 

\begin{figure}[htbp]
    \centering
    \includegraphics[width=8cm]{figs/HQS.pdf}
    \caption{\textbf{Effect of our Hybrid Quality Score (HQS)}. \textbf{Left}: The curve of HQS at different timesteps when the prompt is ``angry". \textbf{Right}: Gradient visualization of the corresponding timestep and editing results of training our image manipulator using only this timestep.}
    \label{HQS}
\end{figure}


Based on this, we propose a timestep selection strategy:
% Before training our image manipulator, we compute the $HQS(\gamma)$ for original images $y \sim q(y)$ at each timestep $t$.

Given text prompt $\gamma$, we compute the $HQS(\gamma)$ at each timestep $t$. Then we build a set of $t$ with a larger $HQS$ value.
Next, when optimizing the image manipulator with Eq.~\eqref{E10}, we sample timesteps $t$ from the set.

To decide the number of timesteps in this set, we introduce a hyperparameter, $\xi$, which controls the tolerance for uncorrelated $t$. While selecting $t$ with the maximum $HQS$ is generally effective, relaxing the HQS requirement can also improve editing. By using a smaller $\xi$, only the most relevant features will change, making the semantic modification relatively simple but requiring fewer optimization costs. On the other hand, using a larger $\xi$ makes the editing more comprehensive but increases the risk of introducing uncorrelated $t$.

In conclusion, training our image manipulator $f_\phi$ with this strategy is shown in Alg. \ref{alg:cap}. 

\begin{algorithm}
\caption{Selective Diffusion Distillation}\label{alg:cap}
\begin{algorithmic}[1]
\State {\bfseries Input:} text prompts $\gamma$, image data $q(y)$, threshold $\xi$, 
 pretrained diffusion model $\epsilon_{\theta}$
\State Compute $\mathrm{HQS}(\gamma)$ by Eq. \eqref{eq:HQS}
\State $S=\{t \mid \mathrm{HQS}_t > \xi \}$
\State Randomly initialize our image manipulator $f_\phi$
\Repeat
    % q0
    \State $y \sim q(y)$, $t \in S$, $\epsilon \sim \mathcal{N}(\mathbf{0},\mathbf{I})$
    \State Take gradient descent step on 
    \State $\qquad \nabla_{\phi}\left \Vert \epsilon - \epsilon_{\theta}(\sqrt{\bar{\alpha}_t}f_\phi(y) + \sqrt{1-\bar{\alpha}_t}\epsilon,t) \right \Vert^2_2$
\Until converged
\end{algorithmic}
\end{algorithm}

Using this strategy leads to a set $S$ of a smaller size. This selected $S$ contains more effective timesteps than the whole timesteps set. Training the image manipulator with selected $S$ finally contributes to faster convergence speed.
We prove the effectiveness in the Sec. \ref{step-selection-exp}. The above analysis is agnostic to the form of our image manipulator so that it can be extended to any image manipulation framework. 

==> legacy/05_experiment.tex <==
\section{Experiments}
\label{sec:experiments}

In this section, we first introduce the details of our framework. 
Then, we compare our method to other image manipulation methods in the aspect of quality and efficiency. 
% 不叫ablation，说清楚一些
After that, we conduct an ablation study on the HQS-based step selection to demonstrate it helps our model capture more semantic. 
% At last, we present our method's qualitative results in a wide range of image manipulation tasks, which shows that our method is general as well as effective.

\subsection{Implementation details}
In the following experiment, we adopt StyleGAN and latent mapper as our image manipulator. Given a source image, we first transfer it into the StyleGAN latent space by using e4e\cite{}. Secondly, the mapper takes the latent to calculate a residual term for editing. Thirdly, we add the residual term to the original latent and give it to the pretrained styleGAN. The styleGAN output image will be passed to the diffusion model. Finally, the diffusion model loss will backpropagate through the computing maps. It is noteworthy that only the mapper's weights are optimized, and all other weights in the diffusion model and styleGAN keep fixed all along the process. 
% ?
The mapper is i  
Overall, this image manipulator strictly follows the configurations in \cite{}. 
For the guidance diffusion model, we employ the latent diffusion \cite{rombach2022stablediffusion}. Besides, regularization losses such as L2 loss\cite{} and ID loss\cite{} are employed to maintain the content of the original images. We also use gradient clipping in some scenarios for training stability.

\subsection{Comparison on editing quality and efficiency}
% baselines
For image editing methods based on the diffusion denoising process, we choose SDEdit \cite{meng2021sdedit} and DDIB \cite{su2022dual} as baselines.
% 0.3 and 0.7
Besides, we also set a baseline that directly borrows the idea from \cite{graikos2022diffusion} and employs it in the image editing task. So we can show our improvements to the diffusion gradient method are non-trivial. We call this method "plug-and-play" for simplicity.

% quality figure here
\begin{figure*}[htbp]
    \includegraphics[width=16cm]{figs/qualitative-v3.pdf}
    \caption{Qualitative results}
    \label{qualitative}
\end{figure*}

\textbf{Qualitative results} As shown in Fig.\ref{qualitative}, our methods significantly overperform these baselines in various image domains and various editing prompts. Existing methods have to trade-off between the realisticity and the editing semantics, while our method keeps both of them. We present more results in our Appendix.

% table of image quality
\begin{table}
    \centering
    \caption{Quantitative results of image quality}
    \label{quantitative}
    \begin{tabular}{lcr}
        \toprule
        Method & FID.   & Time cost\\ 
        \midrule
        DDIB(0.7)                     & 124.067 & -  \\
        DDIB(0.5)                 & 88.321  & -  \\
        DDIB(0.3)                  & 56.226  & -  \\
        SDEdit(0.7)                   & 55.393  & - \\
        SDEdit(0.5)                & 25.062  & - \\
        SDEdit(0.3)                 & 12.231  & - \\
        plug-and-play                & 10.513 & -  \\
        StyleCLIP                    & 16.601  & - \\
        \midrule
        ours-entropy                 & \textbf{5.478} & -   \\
        \bottomrule
    \end{tabular}
\end{table}

\textbf{Quantitative results} To evaluate the realisticity, we take FID \cite{} as the metric. To evaluate the realisticity, we take CLIP \cite{} distance as the metric. The result is shown in Table\ref{quantitative}. It tells that our editing result has the lowest FID and the CLIP distance at the same time. 
For efficiency evaluation, we give a situation that we need to manipulate images to n prompts. For each of the prompts, we have m images to edit. We compute the total inference time cost in this scenario as the metric. 
\begin{equation}
\small
\begin{aligned}
t_{diff} = m \times n \times t_{Unet} \times steps
\end{aligned}
\label{E10}
\end{equation}

\begin{equation}
\small
\begin{aligned}
t_{plug-and-play} =  m \times n \times t_{iter} \times iter 
\end{aligned}
\label{E11}
\end{equation}

\begin{equation}
\small
\begin{aligned}
t_{ours} = n \times t_{iter} \times iter + n \times m \times t_{IM}
\end{aligned}
\label{E12}
\end{equation}

The total time cost of diffusion process methods(DDIB, SDEdit), plug-and-play method, and our method can be formulated as Eq. \eqref{E10}, Eq. \eqref{E11}, and Eq. \eqref{E12} respectively. $t_{Unet}$ denotes the time cost of executing a diffusion Unet. The $steps$ denotes the timesteps required for the diffusion denoising process, which is commonly 1000 in Stable Diffusion. $t_{iter}$ denotes the time of each training iteration in our proposed framework. $iter$ denotes the required iteration for convergence when using diffusion as guidance. $t_{IM}$ denotes the time cost of executing the image manipulator. 
In our method, we need to train individual image manipulators for each of the prompts, and when inference, only the image manipulator is needed.
All of these methods have the complexity of $O(mn)$. However, in our method, the coefficient of $mn$ is $t_{IM}$, which is a much smaller value compared to others.

Empirically, we observe that the $t_{iter}$ is about 1.2x of the $t_{Unet}$, since the image manipulator is much smaller than the Unet. And for the $iter$, when using a proper learning rate, it is 2000 at most. The $t_{IM}$ is approximately $\frac{1}{4}$ of the $t_{Unet}$. 
% deduce diffusion denoising process time cost
When we take our empirical observation to the above equations, we find that when approximately $m > 2.4$, our methods will achieve better efficiency. This efficiency improvement will be exaggerated especially when m becomes larger. The result in the fourth column of Table.\ref{quantitative} shows the real time-cost of these methods. we set m=100, n=5 in the experiment.


\subsection{Experiments entropy-based step selection}
In this section, we conduct experiments on our proposed entropy-based timestep selection. We train the same image manipulator with the same hyperparameters, for the same iterations. The only difference between the experiments is the timestep selection strategy. The "descending" strategy denotes that we choose the descending timesteps along with the training iterations. The "random" strategy \cite{poole2022dreamfusion} denotes that we randomly pick one timestep for each iteration. The "entropy-$x$" strategy denotes that we choose $x$ as the threshold to apply our entropy-based step pruning. The "entropy-best" strategy denotes that we only choose the best timestep according to our entropy metric.

\begin{figure}[htbp]
    \centering
    \includegraphics[width=.5\textwidth]{figs/ablation.pdf}
    \caption{Ablation study on HQS-based timestep selection}
    \label{ablation}
\end{figure}

% baselines: random, descending.
The result in Fig. \ref{ablation} shows that the proposed entropy-based step selection significantly overperforms other baseline methods. The "Descending" and "random" have nearly the same result, and their modification is very small. We attribute this to their redundant timestep selection. The comparison to "fixed\_300" strategy aims to prove that the optimal timesteps of one prompt cannot be transferred to other prompts. Hence searching timesteps for each prompt is necessary. The last column of Fig. \ref{ablation} also shows that different prompts refer to different entropy patterns.
